Gradient-free optimization of highly smooth functions: improved analysis and a new algorithm

This work studies minimization problems with zero-order noisy oracle information under the assumption that the objective function is highly smooth and possibly satisfies additional properties. We consider two kinds of zero-order projected gradient descent algorithms, which differ in the form of the gradient estimator. The first algorithm uses a gradient estimator based on randomization over the $\ell_2$ sphere due to Bach and Perchet (2016). We present an improved analysis of this algorithm on the class of highly smooth and strongly convex functions studied in the prior work, and we derive rates of convergence for two more general classes of non-convex functions. Namely, we consider highly smooth functions satisfying the Polyak-{\L}ojasiewicz condition and the class of highly smooth functions with no additional property. The second algorithm is based on randomization over the $\ell_1$ sphere, and it extends to the highly smooth setting the algorithm that was recently proposed for Lipschitz convex functions in Akhavan et al. (2022). We show that, in the case of noiseless oracle, this novel algorithm enjoys better bounds on bias and variance than the $\ell_2$ randomization and the commonly used Gaussian randomization algorithms, while in the noisy case both $\ell_1$ and $\ell_2$ algorithms benefit from similar improved theoretical guarantees. The improvements are achieved thanks to a new proof techniques based on Poincar\'e type inequalities for uniform distributions on the $\ell_1$ or $\ell_2$ spheres. The results are established under weak (almost adversarial) assumptions on the noise. Moreover, we provide minimax lower bounds proving optimality or near optimality of the obtained upper bounds in several cases.

==> Version_3/section4.tex <==
%!TEX root = main.tex

\section{Upper bounds}\label{sec4}

In this section we present the convergence guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} for various classes of target functions $f$. Each of the following subsections is structured in a similar fashion: first we define the choice of $\eta_t$ and $h_t$ involved in both algorithms and then, for each class of the objective functions, we state the corresponding convergence guarantees.

In Section~\ref{sec:non_convex} we consider the case that $f$ has higher order derivatives, $f \in \mathcal{F}_2(\bar{L}) \cap \mathcal{F}_\beta(L)$ for $\beta \geq 2$, and establish the guarantee for the stationary point. In Section~\ref{sec:non_convex1} we \emph{additionally} assume that $f$ is $\alpha$-gradient dominant and provide guarantees on the optimization error.
In Section~\ref{sec5} we analyze the case of strongly convex target function (both constrained and unconstrained cases), improving the upper bound derived by~\cite{akhavan2020} and~\cite{Gasnikov}.
Unless stated otherwise, the convergence guarantees presented in this section hold under the assumption that the number of queries $T$ is known in before running the algorithms.


\subsection{Only smoothness assumptions}
\label{sec:non_convex}
In this part we only assume that the objective function $f : \bbR^d \to \bbR$ satisfies Assumption~\ref{nat}. In particular, since there is not guarantee of the unicity (or existence) of minimizer, we goal is modest---we only want to obtain a nearly stationary point.

The guarantee of this section will be stated on a randomly sampled point along the trajectory of Algorithms~\ref{algose} or~\ref{algo:simplex}. The distribution on the trajectory is chosen in a careful way, to guarantee the desired convergence.
The distribution that we are going to eventually use is defined in the following lemma.

\begin{lemma}\label{HighSF}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \geq 0$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Assume that $\eta_t$ in Eq.~\eqref{eq:algo_general} is chosen to satisfy $\bL \eta_t m < 1$ and that $f^{\star} > -\infty$.
    Let $S$ be a random variable with values in $\{1, \ldots, T\}$, which is independent from $\bx_1, \ldots, \bx_T, \bg_1, \ldots, \bg_T$ and such that
    \begin{align*}
        \Prob(S = t) = \frac{\eta_t\parent{1 - \bL\eta_tm}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
    Then, it holds that
    \begin{align*}
        \Exp\norm{\nabla f(\bx_S)}^2 \leq \frac{2(\Exp[f(\bx_1)] - f^{\star}) + \sum_{t = 1}^T\eta_t\parent{b_t^2 + \bL\eta_t v_t}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
\end{lemma}
The above lemma, as well as its proof is similar to the techniques used by~\cite{Ghadimi2013} in the context of zero-order non-convex optimization. However, in the work of~\cite{Ghadimi2013} the noise model is different---for them, both $b_t$ and $v_t$ decrease when the discretization parameter $h_t$ ($\mu$ in their notation) decreases.
Note that the distribution of $S$ in Lemma~\ref{HighSF} depends on our choice of $\eta_t$ and $m$. 
In the following result we are going to specify the exact values of $\eta_t$. Meanwhile, the value of $m$ is obtained either from Lemma~\ref{lem:var_sphere_v2} or from Lemma~\ref{lem:var_l1_v2}, depending on the choice of the algorithm.

The next result, as all other results of this section, require a definition of algorithm dependent parameters, which are needed as an input of our algorithms
\begin{align}
    \label{eq:constants_only_smoothness}
    (\mathfrak{y}, \mathfrak{h})
    % (\mathfrak{h}, \mathfrak{n})
    = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 1}{4\beta - 2}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
We recall that $\bar{\tC}_{d,1}$ is the constant which appears and is explicitly defined in Lemma~\ref{lem:var_l1_v2}.

\begin{theorem}\label{nonc}
Let Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algose} or \ref{algo:simplex}, with parameterization $\eta_t$ and $h_{t}$ defined for $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t =\min\left(\frac{\mathfrak{y}}{d},\, d^{-\frac{2(\beta-1)}{2\beta-1}}T^{-\frac{\beta}{2\beta-1}}\right) \qquad\text{and}\qquad 
    h_t = \mathfrak{h}\cdot T^{-\frac{1}{2(2\beta-1)}} \enspace.
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_only_smoothness} depending on the algorithm.
% as: $(\mathfrak{y}, \mathfrak{h}) = \big(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\big)$ for Algorithm~\ref{algose}; $(\mathfrak{y}, \mathfrak{h}) =  \big(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 1}{2\beta - 1}}\big)$ for Algorithm~\ref{algo:simplex}.
% \begin{align*}
%     (\mathfrak{y}, \mathfrak{h}) = 
%     \begin{cases}
%     \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)
%     &\qquad\text{for Algorithm~\ref{algose}}\\
%     % \\
%     \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 2}{2(2\beta - 1)}}\bigg)
%     &\qquad\text{for Algorithm~\ref{algo:simplex}}
%     \end{cases}\enspace.
% \end{align*}
% \begin{align*}
%     \underbrace{(\mathfrak{y}, \mathfrak{h}) = \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)}_{\text{ for Algorithm~\ref{algose}}}\qquad\text{and}\qquad \underbrace{(\mathfrak{y}, \mathfrak{h}) =  \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 2}{2(2\beta - 1)}}\bigg)}_{\text{Algorithm~\ref{algo:simplex}}}\enspace.
% \end{align*}
Assume that $\com = \mathbb{R}^d$, $\bx_{1}$ is deterministic, and $T\geq d^{\frac{1}{\beta}}$, then for $\bx_S$ defined in Lemma~\ref{HighSF} we have
\begin{align*}
     \Exp\norm{\nabla f(\bx_S)}^2 \leq  \Big(\cst_1(f(\bx_1)-f^\star)+\cst_2\Big)\cdot\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{2\beta-1}},
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$, $\beta$, and the choice of the Algorithm.
\end{theorem}


\subsection{Smoothness and \texorpdfstring{$\alpha$}{}-gradient dominance}
\label{sec:non_convex1}
In this section, besides always present Assumption~\ref{nat}, we assume that the objective function $f : \bbR^d \to \bbR$ satisfies the $\alpha$-gradient dominant condition. Importantly, this additional assumption ensures that every stationary point of $f$ is, in fact, its global minimizer~\cite[see e.g.,][]{10.1007/978-3-319-46128-1_50}.


Furthermore, unlike the previous section, here we provide a guarantee on the last point $\bx_T$ along the trajectory of Algorithms~\ref{algose} and~\ref{algo:simplex}. As in the previous subsection, we first define algorithm specific parameters
\begin{align}
    \label{eq:constants_PL}
    (\mathfrak{y}, \mathfrak{h}) = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 2}{2\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
Note that the parameter $\mathfrak{y}$ remains the same as in the previous section, while $\mathfrak{h}$ is modified.
Equipped with the above defined parameters, we can state the main result of this section. 
\begin{theorem}
\label{thm:final_PL}
Let $f: \bbR^d \to \bbR$ be an $\alpha$-gradient dominant function and Assumptions \ref{nat}, \ref{ass1} hold. Consider Algorithm \ref{algose} or~\ref{algo:simplex} with parametrization $\eta_t$ and $h_t$ defined for all $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t = \min\left(\frac{\mathfrak{y}}{d},\, \frac{4}{\alpha t}\right)
    \qquad\text{and}\qquad
    h_t = 
    \mathfrak{h} \cdot \begin{cases}
        t^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{4}{\alpha t}$}\\
        T^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{\mathfrak{y}}{d}$}
    \end{cases}\enspace,
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_PL} depending on the algorithm.
Assume that $\com = \bbR$, $\bx_1$ is deterministic, and ${\color{black}T \geq d^{2-\frac{\beta}{2}}}$, then
\begin{align*}
    \Exp[f(\bx_T)-f^\star] \leq \cst_1\cdot\frac{d }{\alpha T}(f(\bx_1)-f^\star)+\cst_2\cdot\frac{1}{\min\{\alpha,\alpha^2\}}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}},
\end{align*}
where $\cst_{1}, \cst_2>0$ depend only on $\sigma^2, L , \bar{L}$, $\beta$, and the choice of the Algorithm.
\end{theorem}
In the context of deterministic first-order optimization, such condition allows to obtain rates of converges of gradient descent algorithm, which are similar to the case of strongly convex objective function with Lipschitz gradient (this rate is often called linear in the optimization literature~\cite[see e.g.,][]{10.1007/978-3-319-46128-1_50}). Hence, it is natural to expect that on our context the $\alpha$-gradient dominance leads to the same convergence rates as $\alpha$-strong convexity. Unfortunately, the rates established in Theorem~\ref{thm:final_PL} are inflated by a multiplicative factor $\alpha^{-1}$ compared to the strongly convex case that will be discussed in the next section.


Both guarantees (for both algorithms) above rely on the following elementary lemma.

\begin{lemma}
    \label{lem:general}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist three positive sequences $b_t, v_t, m : \bbN \to [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    If $f \in \mathcal{F}_2(\bar{L})$, then for all $t \geq 1$ we have
    \begin{align*}
        \Exp[ f(\bx_{t+1})] \leq \Exp[ f(\bx_{t})] - \frac{\eta_t}{2}\parent{1 - \bL\eta_tm}\Exp\norm{\nabla f(\bx_t)}^2 + \frac{\eta_t}{2}\parent{b_t^2 + \bL\eta_t v_t}\enspace.
    \end{align*}
    
\end{lemma}
Our choices of parameters $\eta_t, h_t > 0$ ensure that $(1 - \bar{L}\eta_t m) > 0$, hence allowing to use the $\alpha$-gradient dominance of the objective function $f$ to relate the norm of the gradient to the optimization error.

As a side remark, we note that by summing up all the inequalities in Lemma~\ref{lem:general} for $t \leq T$ and using the fact that $f(\bx_{T + 1}) \geq f^{\star}$ we arrive at Lemma~\ref{HighSF}, which we used to derive the guarantees in case of smooth functions without additional assumptions (Theorem~\ref{nonc}).

\subsection{Smoothness and strong convexity}\label{sec5}
In this section, we provide the guarantee on the average point $\bar{\bx}_T$ along the trajectory of the algorithm, that is,
\[
    \bar{\bx}_T= \frac{1}{T}\sum_{t = 1}^T \bx_t\enspace.
\]
Note that instead of taking the average along the trajectory one may simply sample uniformly at random one point along the trajectory and our guarantees still hold. However, to avoid additional randomness, we stick to the deterministic averaging.

\subsubsection{Unconstrained optimization}
In this part we consider the case of $\com = \bbR^d$ and, as in the previous parts, we assume that $T$ is known beforehand. The results are presented separately for $\ell_2$ and $\ell_1$-randomizations and the proof strategy is sketched in the end of this subsection.
Analogously to the previous sections, we start with the definition of algorithm dependent constants:
\begin{align}
\label{eq:constants_strongly_convex_unconstrained}
    (\mathfrak{y}, \mathfrak{h}) = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 2}{2\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
% The main result of this section is the convergence 
\begin{theorem}\label{thm:sconvex_uncons}
Let $f$ be an $\alpha$-strongly convex function and Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algose} or \ref{algo:simplex}, with parameterization $\eta_t$ and $h_{t}$ defined for $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t =\min\left(\frac{\alpha \mathfrak{y}}{d},\, \frac{4}{\alpha t}\right) \qquad\text{and}\qquad 
    h_t = 
    \mathfrak{h} \cdot \begin{cases}
        t^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{4}{\alpha t}$}\\
        T^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{\alpha \mathfrak{y}}{ d}$}
    \end{cases} \enspace,
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_strongly_convex_unconstrained} depending on the algorithm.
Assume that $\com = \mathbb{R}^d$, $\bx_{1}$ is deterministic, and $T\geq d^{2 - \frac{\beta}{2}}$, then
\begin{align*}
     \Exp[f(\bar{\bx}_T)-f^*] \leq \cst_1\cdot\frac{d}{\alpha T}\norm{\bx_1-\bx^*}^{2}+\cst_2\cdot\frac{1}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}\enspace,
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$, $\beta$ and the choice of the Algorithm.
\end{theorem}
Note that in the above result, we do not need to impose any condition on $\alpha$. While a similar result in \cite{akhavan2020} suffers from such condition on $\alpha$ forcing this parameter to be larger than a certain threshold.
\paragraph{Proof strategy.}
For the case of $\com = \bbR^d$, the above theorem is based on the following result, which is valid for a rather general class of gradient estimates.

\begin{lemma}\label{scuntunc}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general}.
    Assume that $f$ is $\alpha$-strongly convex on $\mathbb{R}^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \in (0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2  \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, we have for all $\bx \in \com$
    \begin{align*}
        \Exp[f(\bx_t)-f^{\star}]\leq \frac{r_t-r_{t+1}}{2\eta_t}-\frac{\alpha}{4}r_t+\frac{b_{t}^2}{\alpha}+\frac{\eta_t}{2}\big(v_t+m\Exp\|\nabla f (\bx_t)\|^2\big)\enspace,
    \end{align*}
    where $r_t = \Exp\|\bx_t - \bx^*\|^2$.
    
\end{lemma}

\subsubsection{Constrained optimization}
We now we assume that $\com \subset \bbR^d$ be a compact convex set. Consequently, since $f$ is continuously differentiable, its gradient is bounded on $\com$. This fact allows us to develop any-time results, that is, in the present part we do not require the knowledge of the optimization horizon $T$.
The results of this section are essentially corollaries of the following general result.
\begin{lemma}\label{scunt}
    Let $\com \subset \bbR^d$ be a compact convex set.
    Assume that $f$ is $\alpha$-strongly convex on $\com$ and $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Consider the iterative algorithm in Eq.~\eqref{eq:algo_general}.
    Assume that there exist two positive sequences $b_t, v_t,  : \bbN \to [0, \infty)$ and $m \in [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2\leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, for $\bar{\bx}_T = \tfrac{1}{T}\sum_{t = 1}^T \bx_t$ we have
    \begin{align*}
    \Exp[f(\bar\bx_T)-f^\star] \leq \frac{mG^2 \log(e T)}{\alpha T}+ \frac{1}{\alpha T}\sum_{t=1}^{T}\left(\frac{v_t}{t}+b_t^2\right)\enspace.
\end{align*}

\end{lemma}
Using the bounds on the variance and bias derived in Section~\ref{sec3}, we can deduce the following two guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} by analysing the resulting recursive relations.



\begin{theorem}\label{thm:sconvex_cons}
Let $f$ be an $\alpha$-strongly convex function and Assumptions \ref{nat} and \ref{ass1} hold. Consider Algorithm~\ref{algose} or~\ref{algo:simplex} with parametrization $\eta_t =\frac{2}{\alpha t}$ and $h_t = \mathfrak{h} \cdot t^{-1/2\beta}$, where the constant $\mathfrak{h}$ equals to $d^{\frac{1}{\beta}}$ for Algorithm~\ref{algose} and to $d^{\frac{2 + \beta}{2\beta}}$ for Algorithm~\ref{algo:simplex}.
% depending on the algorithm as
% \begin{align*}
%     \mathfrak{h} =
%     \begin{cases}
%     d^{\frac{1}{\beta}} &\qquad\text{for Algorithm~\ref{algose}}\\
%     d^{\frac{2 + \beta}{2\beta}} &\qquad\text{for Algorithm~\ref{algo:simplex}}
%     \end{cases}\enspace.
% \end{align*}
Assume that $\com$ is a convex and closed subset of $\mathbb{R}^d$, with $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Then,
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f(\bx)] &\leq \cst_1\cdot\frac{dG^2\log(eT)}{\alpha T} +\cst_2\cdot\frac{1}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}+\cst_3\cdot\frac{d^{1+\frac{2}{\beta}}}{\alpha T}\enspace,
\end{align*}
 with $\cst_1,\cst_2,\cst_3 > 0$ depend only on $\sigma^2, L, \bL, \beta$ and the choice of the Algorithm.
\end{theorem}
The above results are nearly identical and they only differ in the exact values of constants $\cst_1, \cst_2, \cst_3$. Theorem~\ref{thm:sconvex_cons} should be compared to~\cite[Theorem 4.1 and Theorem 5.1]{akhavan2020} and with~\cite[Theorem 1]{Gasnikov}. Note, however, both~\cite{akhavan2020,Gasnikov} work with a slightly different, compared to ours, notion of smoothness (both coincide in case $\beta = 2$, see our Remark~\ref{rem:smoothness}). The term $\tfrac{d^{1+2/\beta}}{T}$, appearing in both results is negligible as long as $T \geq d^{4 - \beta}$, which, in the worst case of $\beta = 2$ means that $T \geq d^2$.
\begin{remark}
Note that the condition on $d, T$ in this part is worse than in all the previously considered cases. Indeed, before we required that $ T \geq d^{2 - \sfrac{\beta}{2}}$, while here we have $T \geq d^{4 - \beta}$. Such an inflated condition is a consequence of the fact that in the present part the results are obtained \emph{without} the knowledge of the optimization horizon $T$, that is, Theorem~\ref{thm:sconvex_cons} gives anytime guarantees. Actually, one can relax the condition $T \geq d^{4 - \beta}$ back to $T \geq d^{2 - \sfrac{\beta}{2}}$ assuming that $T$ is known and allowing $h_t$ to be dependent on $T$ (as we did in Theorem~\ref{thm:sconvex_uncons}). We do not further pursue this development.
\end{remark}


==> Version_before_20_june_2022/section4.tex <==
\section{Upper bounds}\label{sec4}

% \evg[inline]{here I will write a new version of section 4. It is placed in a separate file section4\_new.tex. there is a HUGE mess of labels and references that should be taken care.}
% \evg[inline]{I erased all the comments from this new version of the section. The old version is right after it.}
% \evg[inline]{I DID NOT TAKE CARE OF REFERENCES. THEY SEND YOU TO THE NEXT SECTION. MOST OF IT WILL BE TAKEN CASE AUTOMATICALLY, IF WE REMOVE THE NEXT SECTION.}
In this section we present the convergence guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} for various classes of target functions $f$. Each of the following subsections is structured in a similar fashion: first we define the choice of $\eta_t$ and $h_t$ involved in both algorithms and then, for each class of the objective functions, we state the corresponding convergence guarantees.

In Section~\ref{sec:non_convex} we consider the case that $f$ has higher order derivatives, $f \in \mathcal{F}_2(\bar{L}) \cap \mathcal{F}_\beta(L)$ for $\beta \geq 2$, and establish the guarantee for the stationary point. In Section~\ref{sec:non_convex1} we \emph{additionally} assume that $f$ is $\alpha$-gradient dominant and provide guarantees on the optimization error.
In Section~\ref{sec5} we analyze the case of strongly convex target function (both constrained and unconstrained cases), improving the upper bound derived by~\cite{akhavan2020} and~\cite{Gasnikov}.
Finally, in Section~\ref{sec:quadratic} we study the class of quadratic functions, improving upon results of~\cite{Shamir17}.
Unless stated otherwise, the convergence guarantees presented in this section hold under the assumption that the number of queries $T$ is known in before running the algorithms.


\subsection{Only smoothness assumptions}
\label{sec:non_convex}
In this part we only assume that the objective function $f : \bbR^d \to \bbR$ satisfies Assumption~\ref{nat}. In particular, since there is not guarantee of the unicity (or existence) of minimizer, we goal is modest---we only want to obtain a nearly stationary point.

The guarantee of this section will be stated on a randomly sampled point along the trajectory of Algorithms~\ref{algose} or~\ref{algo:simplex}. The distribution on the trajectory is chosen in a careful way, to guarantee the desired convergence.
The distribution that we are going to eventually use is defined in the following lemma.

\begin{lemma}\label{HighSF}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \geq 0$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Assume that $\eta_t$ in Eq.~\eqref{eq:algo_general} is chosen to satisfy $\bL \eta_t m < 1$ and that $f^{\star} > -\infty$.
    Let $S$ be a random variable with values in $\{1, \ldots, T\}$, which is independent from $\bx_1, \ldots, \bx_T, \bg_1, \ldots, \bg_T$ and such that
    \begin{align*}
        \Prob(S = t) = \frac{\eta_t\parent{1 - \bL\eta_tm}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
    Then, it holds that
    \begin{align*}
        \Exp\norm{\nabla f(\bx_S)}^2 \leq \frac{2(\Exp[f(\bx_1)] - f^{\star}) + \sum_{t = 1}^T\eta_t\parent{b_t^2 + \bL\eta_t v_t}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
\end{lemma}
The above lemma, as well as its proof is similar to the techniques used by~\cite{Ghadimi2013} in the context of zero-order non-convex optimization. However, in the work of~\cite{Ghadimi2013} the noise model is different---for them, both $b_t$ and $v_t$ decrease when the discretization parameter $h_t$ ($\mu$ in their notation) decreases.
Note that the distribution of $S$ in Lemma~\ref{HighSF} depends on our choice of $\eta_t$ and $m$. 
In the following result we are going to specify the exact values of $\eta_t$. Meanwhile, the value of $m$ is obtained either from Lemma~\ref{lem:var_sphere_v2} or from Lemma~\ref{lem:var_l1_v2}, depending on the choice of the algorithm.

The next result, as all other results of this section, require a definition of algorithm dependent parameters, which are needed as an input of our algorithms
\begin{align}
    \label{eq:constants_only_smoothness}
    (\mathfrak{y}, \mathfrak{h})
    % (\mathfrak{h}, \mathfrak{n})
    = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 1}{4\beta - 2}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
We recall that $\bar{\tC}_{d,1}$ is the constant which appears and is explicitly defined in Lemma~\ref{lem:var_l1_v2}.

\begin{theorem}\label{nonc}
Let Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algose} or \ref{algo:simplex}, with parameterization $\eta_t$ and $h_{t}$ defined for $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t =\min\left(\frac{\mathfrak{y}}{d},\, d^{-\frac{2(\beta-1)}{2\beta-1}}T^{-\frac{\beta}{2\beta-1}}\right) \qquad\text{and}\qquad 
    h_t = \mathfrak{h}\cdot T^{-\frac{1}{2(2\beta-1)}} \enspace.
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_only_smoothness} depending on the algorithm.
% as: $(\mathfrak{y}, \mathfrak{h}) = \big(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\big)$ for Algorithm~\ref{algose}; $(\mathfrak{y}, \mathfrak{h}) =  \big(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 1}{2\beta - 1}}\big)$ for Algorithm~\ref{algo:simplex}.
% \begin{align*}
%     (\mathfrak{y}, \mathfrak{h}) = 
%     \begin{cases}
%     \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)
%     &\qquad\text{for Algorithm~\ref{algose}}\\
%     % \\
%     \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 2}{2(2\beta - 1)}}\bigg)
%     &\qquad\text{for Algorithm~\ref{algo:simplex}}
%     \end{cases}\enspace.
% \end{align*}
% \begin{align*}
%     \underbrace{(\mathfrak{y}, \mathfrak{h}) = \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{2\beta - 1}}\bigg)}_{\text{ for Algorithm~\ref{algose}}}\qquad\text{and}\qquad \underbrace{(\mathfrak{y}, \mathfrak{h}) =  \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{2\beta + 2}{2(2\beta - 1)}}\bigg)}_{\text{Algorithm~\ref{algo:simplex}}}\enspace.
% \end{align*}
Assume that $\com = \mathbb{R}^d$, $\bx_{1}$ is deterministic, and $T\geq d^{\frac{1}{\beta}}$, then for $\bx_S$ defined in Lemma~\ref{HighSF} we have
\begin{align*}
     \Exp\norm{\nabla f(\bx_S)}^2 \leq  \Big(\cst_1(f(\bx_1)-f^\star)+\cst_2\Big)\cdot\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{2\beta-1}},
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$, $\beta$, and the choice of the Algorithm.
\end{theorem}


\subsection{Smoothness and \texorpdfstring{$\alpha$}{}-gradient dominance}
\label{sec:non_convex1}
In this section, besides always present Assumption~\ref{nat}, we assume that the objective function $f : \bbR^d \to \bbR$ satisfies the $\alpha$-gradient dominant condition. Importantly, this additional assumption ensures that every stationary point of $f$ is, in fact, its global minimizer~\cite[see e.g.,][]{10.1007/978-3-319-46128-1_50}.


Furthermore, unlike the previous section, here we provide a guarantee on the last point $\bx_T$ along the trajectory of Algorithms~\ref{algose} and~\ref{algo:simplex}. As in the previous subsection, we first define algorithm specific parameters
\begin{align}
    \label{eq:constants_PL}
    (\mathfrak{y}, \mathfrak{h}) = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 2}{2\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
Note that the parameter $\mathfrak{y}$ remains the same as in the previous section, while $\mathfrak{h}$ is modified.
Equipped with the above defined parameters, we can state the main result of this section. 
\begin{theorem}
\label{thm:final_PL}
Let $f: \bbR^d \to \bbR$ be an $\alpha$-gradient dominant function and Assumptions \ref{nat}, \ref{ass1} hold. Consider Algorithm \ref{algose} or~\ref{algo:simplex} with parametrization $\eta_t$ and $h_t$ defined for all $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t = \min\left(\frac{\mathfrak{y}}{d},\, \frac{4}{\alpha t}\right)
    \qquad\text{and}\qquad
    h_t = 
    \mathfrak{h} \cdot \begin{cases}
        t^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{4}{\alpha t}$}\\
        T^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{\mathfrak{y}}{d}$}
    \end{cases}\enspace,
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_PL} depending on the algorithm.
Assume that $\com = \bbR$, $\bx_1$ is deterministic, and ${\color{black}T \geq d^{2-\frac{\beta}{2}}}$, then
\begin{align*}
    \Exp[f(\bx_T)-f^\star] \leq \cst_1\cdot\frac{d }{\alpha T}(f(\bx_1)-f^\star)+\cst_2\cdot\frac{1}{\min\{\alpha,\alpha^2\}}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}},
\end{align*}
where $\cst_{1}, \cst_2>0$ depend only on $\sigma^2, L , \bar{L}$, $\beta$, and the choice of the Algorithm.
\end{theorem}
In the context of deterministic first-order optimization, such condition allows to obtain rates of converges of gradient descent algorithm, which are similar to the case of strongly convex objective function with Lipschitz gradient (this rate is often called linear in the optimization literature~\cite[see e.g.,][]{10.1007/978-3-319-46128-1_50}). Hence, it is natural to expect that on our context the $\alpha$-gradient dominance leads to the same convergence rates as $\alpha$-strong convexity. Unfortunately, the rates established in Theorem~\ref{thm:final_PL} are inflated by a multiplicative factor $\alpha^{-1}$ compared to the strongly convex case that will be discussed in the next section.


Both guarantees (for both algorithms) above rely on the following elementary lemma.

\begin{lemma}
    \label{lem:general}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist three positive sequences $b_t, v_t, m : \bbN \to [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    If $f \in \mathcal{F}_2(\bar{L})$, then for all $t \geq 1$ we have
    \begin{align*}
        \Exp[ f(\bx_{t+1})] \leq \Exp[ f(\bx_{t})] - \frac{\eta_t}{2}\parent{1 - \bL\eta_tm}\Exp\norm{\nabla f(\bx_t)}^2 + \frac{\eta_t}{2}\parent{b_t^2 + \bL\eta_t v_t}\enspace.
    \end{align*}
    
\end{lemma}
Our choices of parameters $\eta_t, h_t > 0$ ensure that $(1 - \bar{L}\eta_t m) > 0$, hence allowing to use the $\alpha$-gradient dominance of the objective function $f$ to relate the norm of the gradient to the optimization error.

As a side remark, we note that by summing up all the inequalities in Lemma~\ref{lem:general} for $t \leq T$ and using the fact that $f(\bx_{T + 1}) \geq f^{\star}$ we arrive at Lemma~\ref{HighSF}, which we used to derive the guarantees in case of smooth functions without additional assumptions (Theorem~\ref{nonc}).

\subsection{Smoothness and strong convexity}\label{sec5}
In this section, we provide the guarantee on the average point $\bar{\bx}_T$ along the trajectory of the algorithm, that is,
\[
    \bar{\bx}_T= \frac{1}{T}\sum_{t = 1}^T \bx_t\enspace.
\]
Note that instead of taking the average along the trajectory one may simply sample uniformly at random one point along the trajectory and our guarantees still hold. However, to avoid additional randomness, we stick to the deterministic averaging.

\subsubsection{Unconstrained optimization}
In this part we consider the case of $\com = \bbR^d$ and, as in the previous parts, we assume that $T$ is known beforehand. The results are presented separately for $\ell_2$ and $\ell_1$-randomizations and the proof strategy is sketched in the end of this subsection.
Analogously to the previous sections, we start with the definition of algorithm dependent constants:
\begin{align}
\label{eq:constants_strongly_convex_unconstrained}
    (\mathfrak{y}, \mathfrak{h}) = 
    \begin{cases}
    \bigg(\frac{1}{8\kappa\bL},\,d^{\frac{1}{\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algose}}\\
    % \\
    \bigg(\frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2},\, d^{\frac{\beta + 2}{2\beta}}\bigg)
    &\qquad\text{for Algorithm~\ref{algo:simplex}}
    \end{cases}\enspace.
\end{align}
% The main result of this section is the convergence 
\begin{theorem}\label{thm:sconvex_uncons}
Let $f$ be an $\alpha$-strongly convex function and Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algose} or \ref{algo:simplex}, with parameterization $\eta_t$ and $h_{t}$ defined for $t = 1, \ldots, T$ as
\begin{align*}
    \eta_t =\min\left(\frac{\alpha \mathfrak{y}}{d},\, \frac{4}{\alpha t}\right) \qquad\text{and}\qquad 
    h_t = 
    \mathfrak{h} \cdot \begin{cases}
        t^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{4}{\alpha t}$}\\
        T^{-\frac{1}{2\beta}} &\text{ if $\eta_t = \sfrac{\alpha \mathfrak{y}}{ d}$}
    \end{cases} \enspace,
\end{align*}
where the pair of constants $(\mathfrak{y}, \mathfrak{h})$ is defined in Eq.~\eqref{eq:constants_strongly_convex_unconstrained} depending on the algorithm.
Assume that $\com = \mathbb{R}^d$, $\bx_{1}$ is deterministic, and $T\geq d^{2 - \frac{\beta}{2}}$, then
\begin{align*}
     \Exp[f(\bar{\bx}_T)-f^*] \leq \cst_1\cdot\frac{d}{\alpha T}\norm{\bx_1-\bx^*}^{2}+\cst_2\cdot\frac{1}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}\enspace,
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$, $\beta$ and the choice of the Algorithm.
\end{theorem}
Note that in the above result, we do not need to impose any condition on $\alpha$. While a similar result in \cite{akhavan2020} suffers from such condition on $\alpha$ forcing this parameter to be larger than a certain threshold.
\paragraph{Proof strategy.}
For the case of $\com = \bbR^d$, the above theorem is based on the following result, which is valid for a rather general class of gradient estimates.

\begin{lemma}\label{scuntunc}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general}.
    Assume that $f$ is $\alpha$-strongly convex on $\mathbb{R}^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \in (0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2  \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, we have for all $\bx \in \com$
    \begin{align*}
        \Exp[f(\bx_t)-f^{\star}]\leq \frac{r_t-r_{t+1}}{2\eta_t}-\frac{\alpha}{4}r_t+\frac{b_{t}^2}{\alpha}+\frac{\eta_t}{2}\big(v_t+m\Exp\|\nabla f (\bx_t)\|^2\big)\enspace,
    \end{align*}
    where $r_t = \Exp\|\bx_t - \bx^*\|^2$.
    
\end{lemma}

\subsubsection{Constrained optimization}
We now we assume that $\com \subset \bbR^d$ be a closed convex set. Consequently, since $f$ is continuously differentiable, its gradient is bounded on $\com$. This fact allows us to develop any-time results, that is, in the present part we do not require the knowledge of the optimization horizon $T$.
The results of this section are essentially corollaries of the following general result.
\begin{lemma}\label{scunt}
    Let $\com \subset \bbR^d$ be a closed convex set. 
    Assume that $f$ is $\alpha$-strongly convex on $\com$ and $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Consider the iterative algorithm in Eq.~\eqref{eq:algo_general}.
    Assume that there exist two positive sequences $b_t, v_t,  : \bbN \to [0, \infty)$ and $m \in [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2\leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, for $\bar{\bx}_T = \tfrac{1}{T}\sum_{t = 1}^T \bx_t$ we have
    \begin{align*}
    \Exp[f(\bar\bx_T)-f^\star] \leq \frac{mG^2 \log(e T)}{\alpha T}+ \frac{1}{\alpha T}\sum_{t=1}^{T}\left(\frac{v_t}{t}+b_t^2\right)\enspace.
\end{align*}

\end{lemma}
Using the bounds on the variance and bias derived in Section~\ref{sec3}, we can deduce the following two guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} by analysing the resulting recursive relations.



\begin{theorem}\label{thm:sconvex_cons}
Let $f$ be an $\alpha$-strongly convex function and Assumptions \ref{nat} and \ref{ass1} hold. Consider Algorithm~\ref{algose} or~\ref{algo:simplex} with parametrization $\eta_t =\frac{2}{\alpha t}$ and $h_t = \mathfrak{h} \cdot t^{-1/2\beta}$, where the constant $\mathfrak{h}$ equals to $d^{\frac{1}{\beta}}$ for Algorithm~\ref{algose} and to $d^{\frac{2 + \beta}{2\beta}}$ for Algorithm~\ref{algo:simplex}.
% depending on the algorithm as
% \begin{align*}
%     \mathfrak{h} =
%     \begin{cases}
%     d^{\frac{1}{\beta}} &\qquad\text{for Algorithm~\ref{algose}}\\
%     d^{\frac{2 + \beta}{2\beta}} &\qquad\text{for Algorithm~\ref{algo:simplex}}
%     \end{cases}\enspace.
% \end{align*}
Assume that $\com$ is a convex and closed subset of $\mathbb{R}^d$, with $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Then,
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f(\bx)] &\leq \cst_1\cdot\frac{dG^2\log(eT)}{\alpha T} +\cst_2\cdot\frac{1}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}+\cst_3\cdot\frac{d^{1+\frac{2}{\beta}}}{\alpha T}\enspace,
\end{align*}
 with $\cst_1,\cst_2,\cst_3 > 0$ depend only on $\sigma^2, L, \bL, \beta$ and the choice of the Algorithm.
\end{theorem}
The above results are nearly identical and they only differ in the exact values of constants $\cst_1, \cst_2, \cst_3$. Theorem~\ref{thm:sconvex_cons} should be compared to~\cite[Theorem 4.1 and Theorem 5.1]{akhavan2020} and with~\cite[Theorem 1]{Gasnikov}. Note, however, both~\cite{akhavan2020,Gasnikov} work with a slightly different, compared to ours, notion of smoothness (both coincide in case $\beta = 2$, see our Remark~\ref{rem:smoothness}). The term $\tfrac{d^{1+2/\beta}}{T}$, appearing in both results is negligible as long as $T \geq d^{4 - \beta}$, which, in the worst case of $\beta = 2$ means that $T \geq d^2$.
\begin{remark}
Note that the condition on $d, T$ in this part is worse than in all the previously considered cases. Indeed, before we required that $ T \geq d^{2 - \sfrac{\beta}{2}}$, while here we have $T \geq d^{4 - \beta}$. Such an inflated condition is a consequence of the fact that in the present part the results are obtained \emph{without} the knowledge of the optimization horizon $T$, that is, Theorem~\ref{thm:sconvex_cons} gives anytime guarantees. Actually, one can relax the condition $T \geq d^{4 - \beta}$ back to $T \geq d^{2 - \sfrac{\beta}{2}}$ assuming that $T$ is known and allowing $h_t$ to be dependent on $T$ (as we did in Theorem~\ref{thm:sconvex_uncons}). We do not further pursue this development.
\end{remark}

\subsection{Quadratic functions}
\label{sec:quadratic}
In this section we consider quadratic functions $f$. More precisely, we assume that the target function belongs to
\begin{align*}
    \mathcal{F}_{\quadr} \triangleq \enscond{f}{f(\bx) = \bx^{\top}\bfA\bx + \bb^{\top}\bx + c\,,\,\,\, \bb \in \colspan(\bfA)}\enspace,
\end{align*}
where $\bfA$ is a symmetric positive semi-definite matrix in $\mathbb{R}^{d \times d}$, $\bb \in \mathbb{R}^d$, $c \in \mathbb{R}$, $\colspan(\bfA)$ is the column span of $\bfA$. The condition of $\bb \in \colspan(\bfA)$ is necessary to ensure that for any $f \in \class{F}_{\quad}$ we have $f^{\star} > - \infty$.
Denote by $\lambda_{\max}(\bfA)$ and $\lambda_{\min}^{\nz}(\bfA)$ the largest and the smallest \emph{non-zero} eigenvalue of $\bfA$, respectively.
Define the effective dimension and the conditioning number of $\bfA$ as
\begin{align*}
    d_{\eff}(\bfA) \triangleq \frac{\tr(\bfA)}{\lambda_{\max}(\bfA)}\qquad\text{and}\qquad \mu(\bfA) \triangleq \frac{\lambda_{\max}(\bfA)}{\lambda_{\min}^{\nz}(\bfA)}\enspace,
\end{align*}
respectively. Note that the definition of the conditioning number differs from the more conventional one, where instead of the division by the smallest non-zero eigenvalue one divides by the smallest eigenvalue. In our case we do not assume that $\bfA$ is strictly positive definite. Hence, we rely on the definition above, which, unlike the conventional one, is always well defined.
Before stating the main result let us specify the choice of  a ``dummy'' kernel $K(\cdot)$ in Algorithms~\ref{algose} and~\ref{algo:simplex}, namely\footnote{For quadratic functions, the kernel and the randomization introduced by $r \in [-1, 1]$ are not necessary. However, in order to keep all the sections harmonized and avoid the introduction of another algorithm, we simply specify the ``dummy'' kernel above.}
\begin{align}
    \label{eq:dummy_kernel}
    K(r) =
    \begin{cases}
    1, &r \geq 0\\
    -1, &r < 0
    \end{cases}\enspace.
\end{align}

\begin{theorem}\label{thm:upper_quadratic}
Assume that $f \in \mathcal{F}_{\quadr}$ and Assumption~\ref{ass1} is satisfied.
Consider Algorithm~\ref{algose} or~\ref{algo:simplex} with $K(\cdot)$ defined in Eq.~\eqref{eq:dummy_kernel} and
\[
\eta_t = \min \parent{\frac{\mathfrak{y}}{\tr(\bfA)},\, \frac{2}{\lambda_{\min}^{\nz}(\bfA) t}}\qquad\text{and}\qquad h_{t} = \mathfrak{h} \cdot\sqrt{\frac{1}{\lambda_{\min}^{\nz}(\bfA)}} \enspace,
\]
where the pair of parameters $(\mathfrak{y}, \mathfrak{h})$ equals to $(1,\,\sqrt{d})$ for Algorithm~\ref{algose} and to $(0.5,\, \sqrt{2}d)$ for Algorithm~\ref{algo:simplex}.
Assume that $\com=\mathbb{R}^d$ and that $\bx_1$ is determisnitic.
Then,
\begin{align*}
    \Exp[f(\bx_T) - f^\star]\leq \frac{d_{\eff}(\bfA)}{\mu^{-1}(\bfA)}\cdot \frac{\cst_1}{T}\left(f(\bx_1) - f^\star + \cst_2\sigma^2\right)\enspace,
\end{align*}
where $(\cst_1, \cst_2) = (4, 8)$ for Algorithm~\ref{algose} and $(\cst_1, \cst_2) = (8, 5)$ for Algorithm~\ref{algo:simplex}.
\end{theorem}
We remark that both bound on this section involve four main parameters. First of all, the bounds scale linearly with the effective dimension $d_{\eff}(\bfA)$ instead of the ambient one $d$, which can be much lower. Secondly, we again emphasize that the notion of the conditioning number $\mu(\bfA)$ that we use is valid for any positive semi-definite matrix $\bfA$. Finally, the derived rate depends linearly on the quality of the initialization as well as the variance. \cite{Shamir13} provided an upper bound for the optimization of quadratic functions which scales as $d^2 / T$. Note, however, \cite{Shamir13} uses a different notion of noise, which is bounded by the squared norm of the query point.

==> archive/main2.tex <==

{\color{red}
For $k \in \bbN \setminus \{0\}$ let $f^{(k)}$ denote the following $k$-linear form 
\begin{align*}
    f^{(k)}(x)[h_1, \ldots, h_k] \triangleq \sum_{|m_1| = \ldots = |m_k| = 1}^d D^{m_1 + \ldots + m_k}f(x) h_1^{m_1} \cdot \ldots \cdot h_k^{m_k}\,,\qquad \forall h^1, \ldots, h^k \in \bbR^d\enspace.
\end{align*}
Additionally for any $k$-linear form $A$ define its norm as
\begin{align*}
    \|A\| \triangleq \sup\enscond{\abs{A[h_1, \ldots, h_k]}}{\|h_j\| = 1\,\,j = 1, \ldots, k}\enspace.
\end{align*}
\begin{lemma}
Assume that $f : \bbR^d \to \bbR$ is such that there exists $\alpha \in [0, 1]$, an integer $\ell \geq 2$, and $L > 0$ such that for all $x, y \in \bbR^d$
\begin{align}
    \norm{f^{(\ell)}(x) - f^{(\ell)}(y)} \leq L \|x - y\|^\alpha \enspace.\label{eq:holder_alternative}
\end{align}
For any $v \in \bbR^d$ with $\|v\| = 1$ consider $g_v(x) \equiv \scalar{v}{\nabla f(x)}$.
Then,
\begin{align*}
    \norm{g^{(\ell - 1)}_v(x) - g^{(\ell - 1)}_v(y)} \leq L \|x - y\|^\alpha\enspace.
\end{align*}
\end{lemma}
\begin{proof}
By definition of $g^{(\ell - 1)}_v$ we have for any $h^1, \ldots, h^{\ell - 1} \in \bbR^d$
\begin{align*}
    g^{(l - 1)}_v(x)[h^1, \ldots, h^{l - 1}]
    &=
    \sum_{i_1, \ldots, i_{\ell - 1} = 1}^d \frac{\partial^{\ell - 1} g_v(x)}{\partial x_{i_1} \ldots \partial x_{\ell-1}} h^1_{i_1} \cdot \ldots \cdot h^{\ell - 1}_{i_{\ell - 1}}\\
    &=
    \sum_{i_1, \ldots, i_{\ell - 1} = 1}^d \frac{\partial^{\ell - 1} }{\partial x_{i_1} \ldots \partial x_{\ell-1}}\parent{\sum_{i_\ell = 1}^d v_{i_\ell} \frac{\partial}{\partial x_{i_\ell}}}f(x) h^1_{i_1} \cdot \ldots \cdot h^{\ell - 1}_{i_{\ell - 1}}\\
    &=
    \sum_{i_1, \ldots, i_{\ell - 1}, i_\ell = 1}^d \frac{\partial^{\ell}  f(x)}{\partial x_{i_1} \ldots \partial x_{\ell-1} \partial x_{i_\ell}} h^1_{i_1} \cdot \ldots \cdot h^{\ell - 1}_{i_{\ell - 1}}v_{i_\ell}\\
    &=
    f^{(\ell)}(x)[h^1, \ldots, h^{\ell - 1}, v]\enspace.
\end{align*}
Hence, for any $x, y \in \bbR^d$ we can write by definition of the norm of a $l{-}1$-linear form
\begin{align*}
    (*) &= \norm{g^{(\ell - 1)}_v(x) - g^{(\ell - 1)}_v(y)}\\
        &= \sup\enscond{\abs{g^{(\ell - 1)}_v(x)[h^1, \ldots, h^{\ell-1}] - g^{(\ell - 1)}_v(y)[h^1, \ldots, h^{\ell-1}]}}{\|h^j\| = 1\,\,j \in [\ell-1]}\\
        &=
        \sup\enscond{\abs{f^{(\ell)}(x)[h^1, \ldots, h^{\ell - 1}, v] - f^{(\ell)}(y)[h^1, \ldots, h^{\ell - 1}, v]}}{\|h^j\| = 1\,\,j \in [\ell-1]}\\
        &\leq
        \sup\enscond{\abs{f^{(\ell)}(x)[h^1, \ldots, h^{\ell - 1}, h^\ell] - f^{(\ell)}(y)[h^1, \ldots, h^{\ell - 1}, h^\ell]}}{\|h^j\| = 1\,\,j \in [\ell]}\\
        &=
        \norm{f^{(\ell)}(x) - f^{(\ell)}(y)} \leq L \|x - y\|^\alpha\enspace.
\end{align*}
The proof is concluded.
\end{proof}

\begin{lemma}
Fix some real $\beta \geq 2$.
Assume that $f : \bbR^d \to \bbR$ satisfies the condition of Eq.~\eqref{eq:holder_alternative} with $l = \floor{\beta}$ and $\alpha = \beta - \floor{\beta}$.
Then, for all $x, y \in \bbR^d$ it holds that
\begin{equation*}
\bigg|f(x)-\sum_{0\le |m|\leq \ell} \frac{1}{m!}D^{m}f(y)(x-y)^{m} \bigg|\leq \frac{L}{\ell!} \|x-y\|^{\beta},
\end{equation*}
\end{lemma}
\begin{proof}
Fix some $x, y \in \bbR^d$. By Taylor's theorem there exists $\zeta_{x, y}$ such that $\norm{\zeta_{x, y} - y} \leq \norm{x - y}$ for which it holds that
\begin{align*}
    f(x) = \sum_{0\le |m|\leq \ell -1} \frac{1}{m!}D^{m}f(y)(x-y)^{m} + \sum_{0\le |m| = \ell} \frac{1}{m!}D^{m}f(\zeta_{x,y})(x-y)^{m}\enspace.
\end{align*}
Thus, we can write
\begin{align*}
    \bigg|f(x)-\sum_{0\le |m|\leq \ell} \frac{1}{m!}D^{m}f(x)(x-y)^{m} \bigg|
    &=
    \abs{\sum_{0\le |m| = \ell} \frac{1}{m!}\left(D^{m}f(\zeta_{x,y}) - D^mf(y)\right)(x-y)^{m}}\\
    &\leq
    \frac{1}{\ell!}\abs{f^{(\ell)}(\zeta_{x, y})[(x - y), \ldots, (x-y)] - f^{(\ell)}(y)[(x - y), \ldots, (x-y)]}\enspace.
\end{align*}
By multilinearity the above is bounded by
\begin{align*}
    \frac{L}{\ell!} \norm{x - y}^{\ell} \norm{\zeta_{x, y} - y}^{\beta - \ell} \leq \frac{L}{\ell!}\norm{x - y}^\beta\enspace.
\end{align*}
\end{proof}
}

==> archive/old_l1_related.tex <==
The main downside of Lemma~\ref{lem:var_l1_v2} lies in the fact that the absolute constants $\tC_3, \tC_4 > 0$ constants are not explicit as they depend on the following concentration result of~\cite{SchechtmanZinn00}: for some absolute constants $\tC_1, \tC_2 >0$
\begin{align}
    \label{eq:SchechtmanZinn00}
    \Prob\parent{\abs{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]} > t} \leq \tC_1 \exp\parent{-\tC_2 \frac{dt}{L}}\qquad \forall t > 0\enspace,
\end{align}
which holds for all $g : \sphere_d^1 \to \bbR$ such that $|g(\bx) - g(\bx')| \leq L \|\bx - \bx'\|$ for all $\bx, \bx' \in \sphere_d^1$.
Probably the best we could hope for is $\tC_1 = 2$ and $\tC_2 = 1/2$ (mimicking the spherical concentration bound) leading to $\tC_4 \leq 22$ and $\tC_3 \leq 7$, which are rather large but not outrageously large.
We also note that given the non-explicit nature of the constants involved in the concentration result recalled above, we opted out from finely tuning $\tC_4$ and $\tC_3$, which most likely can be reduced significantly.
To be more precise, the proof of Lemma~\ref{lem:var_l1_v2} is based on the following result, which we prove in appendix.


\begin{lemma}
    \label{lem:shamir_likel1}
    Assume that $f \in \mathcal{F}_2(\bar L)$, then for all $\bx \in \bbR^d, r \in [-1, 1], h > 0$ we have
    \begin{align*}
        \Exp \left[\big(f(\bx + hr \bzeta^{\diamond}) - \Exp[f(\bx + hr \bzeta^{\diamond}) ]\big)^2\right] \leq \frac{\tC_4 h^2}{d^2}\parent{\frac{\tC_3\bL h}{\sqrt{d}} + \norm{\nabla f(\bx)}}^2\enspace.
    \end{align*}
    where $\tC_4 = \tfrac{2\tC_1 {+} \sqrt{6\tC_1}}{\tC_2^2}$ and $\tC_3 = \sqrt{2} + \tC_2^{-1}(2 + \log(\tC_1))$
    with $\tC_1, \tC_2 > 0$ provided by Eq.~\eqref{eq:SchechtmanZinn00}.
    \end{lemma}

Let us first recall the following result which is due to~\cite[Theorem 3.1]{SchechtmanZinn00}.

\begin{theorem}
\label{thm:SchechtmanZinn}
% []
Let $\bzeta^{\diamond}$ be distributed uniformly on $\sphere_d^1$. Assume that $g : \sphere_d^1 \to \bbR^d$ is $L$-Lipschitz on $\sphere_d^1$, then there exist absolute constants $\tC_1 \geq 1, \tC_2 > 0$ such that for all $t > 0$,
\begin{align*}
    \Prob\parent{\abs{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]} > t} \leq \tC_1 \exp\parent{-\tC_2 \frac{dt}{L}}\enspace.
\end{align*}
\end{theorem}

The next classical result can be found in~\cite[Theorem 7.2]{mattila95}.

\begin{theorem}
\label{thm:extension}
Let $A \subset \bbR^d$. And assume that $g : A \to \bbR$ is $L$-Lipschitz on $A$, then there exists $g^{\ext} : \bbR^d \to \bbR$ such that $\forall \bu \in A$, $ g^{\ext}(\bu) = g(\bu)$ 
and $g^{\ext}$ is $L$-Lipschitz on $\bbR^d$.
\end{theorem}

% \evg[inline]{Ok, not the most elegant result, I agree, but it does improve the variance nevertheless!}

\begin{proof}[Proof of Lemma~\ref{lem:shamir_likel1}]
    First of all we observe using the same argument as in Lemma~\ref{lem:moments_l1} we can write
    \begin{align*}
        \Exp \norm{\bzeta^{\diamond}} = \frac{\Exp\norm{\bW}}{\Exp\norm{\bW}_1}\enspace,
    \end{align*}
    where $\bW = (W_1, \ldots, W_d)$ are \iid $\exp(1)$ random variables. Note that $\Exp\norm{\bW}_1 = d$.
    Furthermore, by Jensen's inequality $\Exp\norm{\bW} \leq \sqrt{2d}$, implying that $\Exp \norm{\bzeta^{\diamond}} \leq \sqrt{\tfrac{2}{d}}$.
    % One the other hand,  .
    Therefore, since $\bu \mapsto \norm{\bu}$ is $1$-Lipshitz we can write using Theorem~\ref{thm:SchechtmanZinn}
    \begin{align}
        \label{eq:shamir_likel1_1}
         \Prob\bigg(\norm{\bzeta^{\diamond}} > \underbrace{\sqrt{\frac{2}{{d}}}+ \frac{\log(d^2 \tC_1)}{\tC_2 d}}_{=: a_d} \bigg) \leq \Prob\parent{\norm{\bzeta^{\diamond}} > \Exp[\norm{\bzeta^{\diamond}}] + \frac{\log(d^2 \tC_1)}{\tC_2 d}} \leq \frac{1}{d^2}\enspace,
    \end{align}
    where we also introduced $a_d : = \sqrt{\tfrac{2}{{d}}} + \tfrac{\log(d^2 \tC_1)}{\tC_2 d}$.
    Introduce, the following set
    \begin{align}
        \label{eq:shamir_likel1_2}
        A = \sphere_d^1 \cap \enscond{\bu \in \bbR^d}{\norm{\bu} \leq a_d}\enspace.
    \end{align}
    We define $g(\bu) = f(\bx + hr \bu)$ for all $\bu \in \sphere_d^1$.
    Noticing that since $f \in \mathcal{F}_2(\bL)$, it holds that $\|\nabla g(\bu)\| = h |r| \| \nabla f(\bx + hr\bu)\| \leq h(\bL h \norm{\bu} + \|\nabla f(\bx)\|)$ for all $\bu \in \sphere_d^1$, we deduce using the mean value theorem that for all $\bu, \bu' \in A$ 
    \begin{equation}
    \label{eq:shamir_likel1_3}
    \begin{aligned}
        \abs{g(\bu) - g(\bu')}
        &\leq
        % h\parent{\bL h \sup_{\bv \in A}\norm{\bv} + \norm{\nabla f (\bx)}} \norm{\bu - \bu'}\\
        % &\leq
        h\parent{\bL h a_d + \norm{\nabla f (\bx)}} \norm{\bu - \bu'}\enspace.
    \end{aligned}
    \end{equation}
    Furthermore, for all $\bu, \bu' \in \sphere_d^1$ we have
    \begin{align}
        \label{eq:shamir_likel1_4}
        \abs{g(\bu) - g(\bu')}
        \leq
        h\parent{\bL h + \norm{\nabla f (\bx)}} \norm{\bu - \bu'}\enspace.
    \end{align}
    Now we are ready to prove the claim of the lemma.
    Consider the following decomposition
    \begin{align*}
        \Exp \parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^2 =  \texttt{T}_1 + \texttt{T}_2\enspace,
    \end{align*}
    where
    \begin{align*}
        \texttt{T}_1 &:= \Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \in A} \right]\qquad\text{and}\qquad
        \texttt{T}_2 := \Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \not\in A}\right]\enspace.
    \end{align*}
    We bound each of these terms separately.
    \paragraph{Bound on $\texttt{T}_1$.} Define $g_A : A \to \bbR$ as the restriction of $g : \sphere_d^1 \to \bbR$ onto $A$. Thanks to Eq.~\eqref{eq:shamir_likel1_3}, $g_A$ is $h\parent{\bL h a_d + \norm{\nabla f (\bx)}}$-Lipschitz on $A$. Consider an extension $g_A^{\ext}$ of $g_A$ onto $\bbR^d$ provided by Theorem~\ref{thm:extension}, which preserves the Lipschitz constant.
    Hence, we can write
    \begin{align*}
        \texttt{T}_1
        :=
        \Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \in A}\right]
        &=
        \Exp\left[\parent{g_A(\bzeta^{\diamond}) - \Exp[g_A(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \in A}\right]\\
        &=
        \Exp\left[\parent{g_A^{\ext}(\bzeta^{\diamond}) - \Exp[g_A^{\ext}(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \in A}\right]\\
        &\leq
        \Exp\left[\parent{g_A^{\ext}(\bzeta^{\diamond}) - \Exp[g_A^{\ext}(\bzeta^{\diamond})]}^2\right]\enspace.
    \end{align*}
    Since, by construction, $g_A^{\ext}$ is $h\parent{\bL h a_d + \norm{\nabla f (\bx)}}$-Lipschitz and using Theorem~\ref{thm:SchechtmanZinn}, we deduce
    \begin{align*}
        \Exp\left[\parent{g_A^{\ext}(\bzeta^{\diamond}) - \Exp[g_A^{\ext}(\bzeta^{\diamond})]}^2\right]
        &\leq
        \tC_1\int_0^{\infty}\exp\parent{- \frac{\tC_2d\sqrt t}{h(\bL h a_d + \norm{\nabla f (\bx)})}} \d t\\
        &=
        \frac{2\tC_1h^2}{\tC_2^2d^2}\parent{\bL h a_d + \norm{\nabla f (\bx)}}^2\enspace.
    \end{align*}
    
    \paragraph{Bound on $\texttt{T}_2$.} Using Cauchy-Schwartz inequality, we obtain
    \begin{align*}
        \texttt{T}_2 := \Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^2\ind{\bzeta^{\diamond} \not\in A}\right]
        \leq
        \sqrt{\Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^4\right]} \sqrt{\Prob(\bzeta^{\diamond} \not\in A)}\enspace.
    \end{align*}
    % Eq.~\eqref{eq:shamir_likel1_1} implies that
    % \begin{align*}
    %     \texttt{T}_2 \leq \frac{1}{d}\sqrt{\Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond}] )}^4\right]}\enspace.
    % \end{align*}
    Due to Eq.~\eqref{eq:shamir_likel1_4}, the function $g$ is $h(\bL h + \norm{\nabla f(\bx)})$-Lipschitz and we again use Theorem~\ref{thm:SchechtmanZinn} to show
    \begin{align*}
        \Exp\left[\parent{g(\bzeta^{\diamond}) - \Exp[g(\bzeta^{\diamond})]}^4\right]
        \leq
        \tC_1\int_{0}^{\infty}\exp\parent{- \frac{\tC_2dt^{1/4}}{h(\bL h + \norm{\nabla f(\bx)})}}\d t
        =
        \frac{24\tC_1h^4}{\tC_2^4 d^4}(\bL h + \norm{\nabla f(\bx)})^4\enspace.
    \end{align*}
    Hence, the above bound in conjunction with Eq.~\eqref{eq:shamir_likel1_1} yields
    \begin{align*}
        \texttt{T}_2
        \leq
        \frac{\sqrt{24\tC_1}h^2}{\tC_2^2 d^3}(\bL h + \norm{\nabla f(\bx)})^2
        &\leq
        \frac{\sqrt{6\tC_1}h^2}{\tC_2^2 d^2}\parent{\bL h\sqrt{\frac{2}{d}} + \norm{\nabla f(\bx)}}^2
        \leq
        \frac{\sqrt{6\tC_1}h^2}{\tC_2^2 d^2}\parent{\bL ha_d + \norm{\nabla f(\bx)}}^2\enspace.
    \end{align*}
    
    We conclude by combining the above derived bounds for $\texttt{T}_1$ and $\texttt{T}_2$ with the observation that
    \begin{align*}
        a_d
        % : = \sqrt{\frac{2}{{d}}} + \frac{\log(d^2 \tC_1)}{\tC_2 d}
        &=
        \frac{1}{\sqrt{d}}\parent{\sqrt{2} + \tC_2^{-1}\parent{{\frac{2\log d}{\sqrt{d}} + \frac{\log(\tC_1)}{\sqrt{d}}}}}
        \leq
        \frac{1}{\sqrt{d}}\parent{\sqrt{2} + \tC_2^{-1}\parent{2 + \log(\tC_1)}} = \frac{\tC_3}{\sqrt{d}}\enspace,
    \end{align*}
    with $\tC_3$ introduced in the statement of the result.
\end{proof}

==> archive/section4_old.tex <==
\section{Upper bounds}\label{sec4}
In this section we present the convergence guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} for various classes of target functions $f$. Each of the following subsections is structured in a similar fashion: first we define the choice of $\eta_t$ and $h_t$ involved in both algorithms and then, for each class of the objective functions, we state the corresponding convergence guarantee.

In Section~\ref{sec:non_convex} we consider the case that $f$ has higher order derivatives, $f \in \mathcal{F}_2(\bar{L}) \cap \mathcal{F}_\beta(L)$ for $\beta \geq 2$, and establish the guarantee for the stationary point. In Section~\ref{sec:non_convex1} we \emph{additionally} assume that $f$ is $\alpha$-gradient dominant and provide guarantees on the optimization error.
In Section~\ref{sec5} we analyze the case of strongly convex target function (both constrained and unconstrained cases), improving the upper bound derived by~\cite{akhavan2020} and~\cite{Gasnikov}.
Finally, in Section~\ref{sec:quadratic} we study the class of quadratic functions, improving upon results of~\cite{Shamir17}.

Unless stated otherwise, in our guarantees of this section we assume that the number of queries $T$ is known beforehand. 


\subsection{Only smoothness assumptions}
\label{sec:non_convex}
In the section we provide a guarantee on a randomly sampled point along the trajectory of Algorithms~\ref{algose} or~\ref{algo:simplex}. The distribution on the trajectory is chosen in a careful way, to guarantee the desired convergence.
The distribution that are going to eventually use is defined in the following lemma.

\begin{lemma}\label{HighSF}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \geq 0$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Assume that $\eta_t$ in Eq.~\eqref{eq:algo_general} is chosen to satisfy $\bL \eta_t m < 1$ and that $f^{\star} > -\infty$.
    Let $S$ be a random variable with values in $\{1, \ldots, T\}$, which is independent from $\bx_1, \ldots, \bx_T, \bg_1, \ldots, \bg_T$ and such that
    \begin{align*}
        \Prob(S = t) = \frac{\eta_t\parent{1 - \bL\eta_tm}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
    Then, it holds that
    \begin{align*}
        \Exp\left[\norm{\nabla f(\bx_S)}^2\right] \leq \frac{2(\Exp[f(\bx_1)] - f^{\star}) + \sum_{t = 1}^T\eta_t\parent{b_t^2 + \bL\eta_t v_t}}{\sum_{t = 1}^T\eta_t\parent{1 - \bL\eta_tm}}\enspace.
    \end{align*}
\end{lemma}
\massi[inline]{Let's discuss whether we can expland this discussion a little}
Note that the distribution of $S$ in Lemma~\ref{HighSF} depends on our choice of $\eta_t$ and $m$. 
While in the following results we are going to specify the exact values of $\eta_t$, the value of $m$ are obtained from Lemma~\ref{lem:var_sphere_v2} and Lemma~\ref{lem:var_l1_v2}.

\begin{restatable}[$\ell_2$-randomization]{theorem}{nc}\label{nonc}
Let Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algose}, with parameterization $\eta_t$ and $h_{t}$ defined for $t = 1, \ldots, T$ as
\begin{align}
\label{par21}
    {\color{purple}\eta_t =\min\left(\frac{m_{\ell_2}}{d},\, d^{-\frac{2(\beta-1)}{2\beta-1}}T^{-\frac{\beta}{2\beta-1}}\right)} \qquad\text{and}\qquad 
    h_t = \left(\frac{d^2}{T}\right)^{\frac{1}{2(2\beta-1)}} \enspace,
\end{align}
$\com = \mathbb{R}^d$ and non random $\bx_{1}$, {\color{purple}with $m_{\ell_2} = \frac{1}{8\kappa\bL}$}. If {\color{black}$T\geq d^{\frac{1}{\beta}}$}, then for $\bx_S$ defined in Lemma~\ref{HighSF} we have
\begin{align*}
     \Exp\left[\norm{\nabla f(\bx_S)}^2\right] \leq  \Big(\cst_1(f(\bx_1)-f^\star)+\cst_2\Big)\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{2\beta-1}},
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$ and $\beta$.
\end{restatable}

\begin{theorem}[$\ell_1$-randomization]\label{nonc:simp}
Let Assumptions \ref{nat} and \ref{ass1} hold, for $\beta\geq2$. Consider Algorithm \ref{algo:simplex}, with parameterization $\eta_t$ and $h_t$ defined for $t = 1,\ldots, T$ as
\begin{align}
\label{par21}
    {\color{purple}\eta_t =\min\left(\frac{m_{\ell_1}}{d},\,d^{-\frac{2(\beta-1)}{2\beta-1}}T^{-\frac{\beta}{2\beta-1}}\right)}
    \quad\text{and}\quad
    h_t = d^{\frac{2\beta+1}{2(2\beta-1)}}T^{-\frac{1}{2(2\beta-1)}}\enspace,
\end{align}
$\com = \mathbb{R}^d$ and non random $\bx_{1}$, {\color{purple}with $m_{\ell_1} = \frac{(d-2)(d-1)}{2\bL\bar{\tC}_{d,1} d^2}$}. If ${\color{black}T\geq d^\frac{1}{\beta}}$, then for $\bx_S$ defined in Lemma~\ref{HighSF} with we have
\begin{align*}
     \Exp\left[\norm{\nabla f(\bx_S)}^2\right] \leq  \Big(\cst_1(f(\bx_1)-f^\star)+\cst_2\Big)\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{2\beta-1}},
\end{align*}
where the constants $\cst_1, \cst_2>0$ depend only on $\sigma, L, \bar{L}$ and $\beta$.
\end{theorem}
\massi[inline]{The subsection ends without any comment on these two theorems. Let's talk}


\subsection{Smoothness and \texorpdfstring{$\alpha$}{}-gradient dominance}
\label{sec:non_convex1}
In this section we assume that the total number of iterations $T$ is known beforehand. \massi[inline]{A bit unclear as you already said that at the end of sect. 4.1}
In other words, the final guarantee is \emph{not} any time. However, unlike the previous section, here we provide a guarantee on the last point $\bx_T$ along the trajectory of Algorithms~\ref{algose} and~\ref{algo:simplex}.

% For $\alpha$-gradient dominant functions, the main idea of the proof is to use Lemma \ref{golden} and use the bound 
% $2\alpha(f(x) - f^*) \leq \norm{\nabla f(x)}^2$,
% with $f^*=\min_{x \in \mathbb{R}^d}f(x)$, which comes from Definition \ref{PL}. 


\massi[inline]{in this and the next subsection I would put the conditions on $\ell_2$ and $\ell_1$ randomization inside Theorems 17 and 18, respectively}
\paragraph{For \texorpdfstring{$\ell_2$}{}-randomization.}
% \label{sec:PL_smooth}
% First we assign the parameters $\eta_t$ and $h_t$ for $t=1,\dots,T$.
Let us define ${\color{purple}T_0 = \floor{\frac{4d}{m_{\ell_2}\alpha}}}$ and for all $t \geq 1$ we set
\begin{align*}
    {\color{purple}\eta_t = \min\left(\frac{m_{\ell_2}}{d},\, \frac{4}{\alpha t}\right)}
    \qquad\text{and}\qquad
    h_t = 
    \begin{cases}
        \Big(\frac{d^2}{t}\Big)^{\frac{1}{2\beta}} &t \in [T_0+1, T]\\
        \Big(\frac{d^2}{T}\Big)^{\frac{1}{2\beta}} &t \in [1, T_0]
    \end{cases}\enspace,
\end{align*}
with {\color{purple}$m_{\ell_2} = \frac{1}{8\kappa \bL}$}, and the agreement that $[T_0 + 1, T] = \emptyset$ for all $T \leq T_0$.
% \evg[inline]{Here I erased the splitting, which looked weird and seemed to be applied by the above. To discuss.}
% If $T \leq T_0$, then we set
% \begin{align*}
%     \eta_t = \frac{1}{18\kappa\bL d}
%     \qquad\text{and}\qquad
%     h_t = \Big(\frac{d^2}{T}\Big)^{\frac{1}{2\beta}}\enspace.
% \end{align*}


% For $t \leq T_0$, let $h_t = \Big(\frac{d^2}{T}\Big)^{\frac{1}{2\beta}}$, and in the case that $T_0\leq T$, for any $t>T_0$ let $h_t = \Big(\frac{d^2}{t}\Big)^{\frac{1}{2\beta}}$. Also, let $\eta_t = \Big(\frac{1}{18\kappa\bL d}, \frac{4}{\alpha t}\Big)$, for $t =1,\dots,T$. It is clear that, for $t \leq T_0$ we have $\eta_t = \frac{1}{18\kappa\bL d}$ and for $T_0\leq t$ we have $\eta_t = \frac{4}{\alpha t}$.

\massi[inline]{1. to discuss a moment if we can combine the two thms in a single one. 2.strage sentence in the thms: "with."}


\begin{restatable}{theorem}{ploptgoo}\label{plgoo}
Let $f$ be an $\alpha$-gradient dominant function. Consider the above parameterization, for Algorithm \ref{algose} with. Let Assumptions \ref{nat} and \ref{ass1} hold, and assume that $\bx_1$ is non-random.  %$\in \com$ 
If ${\color{black}T \geq d^{2-\frac{\beta}{2}}}$, then 
\begin{align}
    \Exp[f(\bx_T)-f^\star] \leq \cst_1\frac{d }{\alpha T}(f(\bx_1)-f^\star)+\frac{\cst_2}{\min\{\alpha,\alpha^2\}}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}},
\end{align}
where $\cst_{1}, \cst_2>0$ depend only on $\sigma^2, L , \bar{L}$, and $\beta$.
\end{restatable}

\paragraph{For \texorpdfstring{$\ell_1$}{}-randomization.}
Let us define ${\color{purple}T_0 = \floor{\frac{4d}{m_{\ell_1}\alpha}}}$. For all $t \geq 1$ we set
\begin{align*}
    {\color{purple}\eta_t = \min\left(\frac{m_{\ell_1}}{d},\, \frac{4}{\alpha t}\right)}\qquad\text{and}\qquad 
    h_t = 
    \begin{cases}
        d^{\frac{2+\beta}{2\beta}}t^{-\frac{1}{2\beta}} &t \in [T_0+1, T]\\
        d^{\frac{2+\beta}{2\beta}}T^{-\frac{1}{2\beta}} &t \in [1, T_0]
    \end{cases}\enspace.
    % h_t &= d^{\frac{2+\beta}{2\beta}}t^{-\frac{1}{2\beta}},\quad \text{for  } T_0+1\leq t\leq T\\
    % h_t &= d^{\frac{2+\beta}{2\beta}}T^{-\frac{1}{2\beta}}, \quad \text{for  } 1\leq t \leq T_0
\end{align*}
where {\color{purple}$m_{\ell_1} = \frac{(d-2)(d-1)}{2\bL{\bar{\tC}}_{d,1}d^2\kappa }$}, and again with the agreement that $[T_0 + 1, T] = \emptyset$ for all $T \leq T_0$.
% If $T \leq T_0$, then we set
% \begin{align*}
%     \eta_t = \frac{1}{16\bL\kappa d}\qquad\text{and}\qquad h_t = d^{\frac{2+\beta}{2\beta}}T^{-\frac{1}{2\beta}}\enspace.
% \end{align*}
% $$ and $h_t = d^{\frac{2+\beta}{2\beta}}T^{-\frac{1}{2\beta}}$, for $1 \leq t \leq T$.
\begin{theorem}\label{plgoo:simplex}
Let $f$ be an $\alpha$-gradient dominant function. Consider the above parameterization, for Algorithm \ref{algo:simplex} with. Let Assumptions \ref{nat} and \ref{ass1} hold, and assume that $\bx_1$ is non-random.   %$\in \com$ 
If ${\color{black}T \geq d^{2-\frac{\beta}{2}}}$, then 
\begin{align*}
    \Exp[f(\bx_T)-f^\star] \leq \cst_1\frac{d }{\alpha T}(f(\bx_1)-f^\star)+\frac{\cst_2}{\min\{\alpha,\alpha^2\}}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}},
\end{align*}
where $\cst_{1}, \cst_2>0$ depend only on $\sigma^2, L , \bar{L}$, and $\beta$.
\end{theorem}


\paragraph{Proof strategy.} Both results of this part rely on the following elementary lemma.

\begin{lemma}
    \label{lem:general}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general} with $\com = \bbR^d$.
    Assume that there exist three positive sequences $b_t, v_t, m : \bbN \to [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2 \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    If $f \in \mathcal{F}_2(\bar{L})$, then for all $t \geq 1$ we have
    \begin{align*}
        \Exp[ f(\bx_{t+1})] \leq \Exp[ f(\bx_{t})] - \frac{\eta_t}{2}\parent{1 - \bL\eta_tm}\Exp\left[\norm{\nabla f(\bx_t)}^2\right] + \frac{\eta_t}{2}\parent{b_t^2 + \bL\eta_t v_t}\enspace.
    \end{align*}
    
\end{lemma}
Our choices of parameters $\eta_t, h_t > 0$ ensure that $(1 - \bar{L}\eta_t m) > 0$, hence allowing to use the $\alpha$-gradient dominance of the objective function $f$ to relate the norm of the gradient to the optimization error.
Summing up all the inequalities in Lemma~\ref{lem:general} for $t \leq T$ and using the fact that $f(\bx_{T + 1}) \geq f^{\star}$ we arrive at Lemma~\ref{HighSF}, \massi[inline]{strange to refer to Lemma 13 which is in the previous section} which we used to derive the guarantees in case of smooth functions without additional assumptions (Theorems~\ref{nonc} and~\ref{nonc:simp}).


\begin{comment}
\textcolor{red}{In the next theorem we show the performance of Algorithm \ref{algo:grad}, for the functions which satisfies $\alpha$-restricted secant inequality.}
\begin{restatable}{theorem}{rsintheorem}\label{rsi}
Let $f$ satisfies $\alpha$-restricted secant inequality. Consider $\eta_{t} = \min (\frac{\alpha}{18\bar{L}^2\kappa}, \frac{1}{\alpha t})$, and $h_{t} = t^{-\frac{1}{2\beta}}$, for Algorithm \ref{algo:grad} with $\com = \mathbb{R}^d$, and assume that $x_{1}$ is non-random. Let Assumptions \ref{nat} and \ref{ass1} hold. If $\sigma > 0$, then for any $x^* \in \argmin_{x \in \mathbb{R}^d}f(x)$, we have 
\begin{align*}
    \Exp[f(\bx_{T}) - f(x^*)]\leq \frac{\bar{L}\norm{x_1 -x_{p}}^2}{2T}+\mathcal{C}\frac{d}{\alpha^2}T^{-\frac{\beta-1}{\beta}}
\end{align*}
where $\mathcal{C}>0$ depends only on $\sigma^2, L, \bar{L}$, and $\beta$.
\end{restatable}
\textcolor{red}{Theorem \ref{crsi}, is the constrained version of Theorem \ref{rsi}, where $\com$ in Algorithm \ref{algo:grad}, is a compact convex subset of $\mathbb{R}^d$ which contains a global minimzer of $f$.}
\begin{restatable}{theorem}{rsitheorem}\label{crsi}
Let $f$ satisfies $\alpha$-restricted secant inequality. Consider $\eta_{t} = \frac{1}{\alpha t}$, and $h_{t} = t^{-\frac{1}{2\beta}}$, for Algorithm \ref{algo:grad} with $\max_{x,y \in \com}\norm{x-y}^2\leq B<\infty$. Let Assumptions \ref{nat} and \ref{ass1} hold. If $\sigma > 0$, then for any $x^* \in \argmin_{x \in \mathbb{R}^d}f(x)\cap \com$, we have
\begin{align*}
   \Exp[f(x_{T}) - f(x^*)]\leq \frac{\bar{L}B}{2T}+\mathcal{C}\frac{d}{\alpha^2}T^{-\frac{\beta-1}{\beta}},
\end{align*}
where $\mathcal{C}>0$ depends only on $\sigma^2, L, \bar{L}$, and $\beta$.
\end{restatable}


%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{restatable}{theorem}{evgoo}\label{evgoo}
Let $f$ be an $\alpha$-gradient dominant function. Consider $\eta_{t} = \min\left(\tfrac{1}{18L\kappa}, \tfrac{2}{\alpha t}\right)$, and $h_{t} = t^{-\frac{1}{2\beta}}$, for Algorithm \ref{algose} with $\com=\mathbb{R}^d$, and assume that $\bx_1$ is deterministic. Let Assumptions \ref{nat}(ii) and \ref{ass1} hold, and assume that $f$ is $(\beta, L)$-H\"older. %$\in \com$ 
Then, if $T \geq d^2$ we have
\begin{align}
    \Exp[f(\bx_T)-f^*] \leq  \cst_1\frac{d}{T\alpha}\Big(f(\bx_1)-f^*\Big) + \frac{\cst_{2}}{\min\{\alpha, \alpha^2\}}\big(\frac{d^2}{T}\big)^{\frac{\beta-1}{\beta}},
\end{align}
where $\cst_{5}>0$ depends only on $\sigma^2, L , \bar{L}$, and $\beta$.
\end{restatable}

\end{comment}

\subsection{Smoothness and strong convexity}\label{sec5}
%Consider the iterative algorithm described in Eq.~\eqref{eq:algo_general}, with $\bg_t$ being built upon $\ell_2$ or $\ell_1$-randomizations.
In this section, we provide the guarantee on the average point $\bar{\bx}_T$ along the trajectory of the algorithm, that is,
\[
    \bar{\bx}_T= \frac{1}{T}\sum_{t = 1}^T \bx_t\enspace.
\]
Note that instead of taking the average along the trajectory one may simply sample uniformly at random one point along the trajectory and our guarantees still hold. However, to avoid additional randomness, we stick to the deterministic averaging.

\massi[inline]{comment why for alpha-GD we do not get results for the average? (or we do?) in general we may want to comment, at the beginning of sec. 4 and the introduction, about the different flavours of the results (random $x_t$, last iterate, average) and what this implies}

\subsubsection{Unconstrained optimization}
In this part we consider the case of $\com = \bbR^d$ and, as in the previous parts, we assume that $T$ is known beforehand. The results are presented separately for $\ell_2$ and $\ell_1$-randomizations and the proof strategy is sketched in the end of this subsection.

\paragraph{For \texorpdfstring{$\ell_2$}{}-randomization.}
% \arya[inline]{First I wrote the proof, then I found a mistake in controlling $T_3$ in the proof and the line that I wrote for this is wrong. For now, consider this section undone.}
% First we assign the parameters $\eta_t$ and $h_t$ for $t=1,\dots,T$.
Denote {\color{purple}$T_0 = \floor{\frac{4d}{m_{\ell_2}\alpha^2}}$} and for all $t \geq 1$ we set
\begin{align*}
    \eta_t = \min\left({\color{purple}{\frac{\alpha m_{\ell_2}}{d}}},\, \frac{4}{\alpha t}\right)
    \qquad\text{and}\qquad
    h_t = 
    \begin{cases}
        \Big(\frac{d^2}{t}\Big)^{\frac{1}{2\beta}} &t \in [T_0+1, T]\\
        \Big(\frac{d^2}{T}\Big)^{\frac{1}{2\beta}} &t \in [1, T_0]
    \end{cases}\enspace,
\end{align*}
with {\color{purple}$m_{\ell_2} = \frac{1}{8\kappa \bL}$}, and the agreement that $[T_0 + 1, T] = \emptyset$ for all $T \leq T_0$.


\begin{theorem}[$\ell_2$-randomization]
\label{thm:sconvex_l2_uncons}
Let $f$ be an $\alpha$-strongly convex function. Consider the above parametrization for Algorithm \ref{algose}, and assume that $\bx_1$ is non-random. Let Assumptions \ref{nat} and \ref{ass1} hold. If {${\color{black}T \geq d^{2-\frac{\beta}{2}}}$}, then  
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f^*] \leq \cst_1\frac{d}{\alpha T}\norm{\bx_1-\bx^*}^{2}+\frac{\cst_2}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}\enspace,
\end{align*}
 with $\cst_1,\cst_2 > 0$ depend only on $\sigma^2, L, \bL, \beta$.
\end{theorem}

\begin{comment}
For the sake of comparison, for Theorems \ref{plgoo} and \ref{thm:2}, we have the bound of the order $\frac{d^{2-\frac{1}{\beta}}}{\alpha^2}T_{0}^{-\frac{\beta-1}{\beta}}$, and $\frac{d^{2-\frac{1}{\beta}}}{\alpha}T_{0}^{-\frac{\beta-1}{\beta}}$, respectively. Here, we have the improvement with respect to the parameter $d$, where in the previous works [I need to mention references here] the dependency is of the order $d^2$. Note that in Theorem \ref{thm:2}, we do not need to impose any condition on $\alpha$. While a similar result in \cite{akhavan2020} suffers from this condition on $\alpha$, which forces this parameter to be larger than some certain threshold.

Now, we provide the results of constrained optimization, for $\alpha$-strongly convex functions, where $\com$ is a convex compact subset of $\mathbb{R}^d$. First, we apply Algorithm \ref{algo:grad} for $\beta \geq 2$, and obtain the upper bounds for both online regret and optimization error. Later by a different approach we show a finer result for the case $\beta = 2$.
\end{comment}
\paragraph{For \texorpdfstring{$\ell_1$}{}-randomization.}
Denote {\color{purple}$T_0 = \floor{\frac{4d}{m_{\ell_1}\alpha^2}}$} and for all $t \geq 1$, we set
\begin{align*}
    \eta_t = \min\left({\color{purple}{\frac{\alpha m_{\ell_1}}{d}}},\, \frac{4}{\alpha t}\right)
    \qquad\text{and}\qquad
    h_t = 
    \begin{cases}
        d^{\frac{2+\beta}{2\beta}}t^{-\frac{1}{2\beta}} &t \in [T_0+1, T]\\
        d^{\frac{2+\beta}{2\beta}}T^{-\frac{1}{2\beta}} &t \in [1, T_0]
    \end{cases}\enspace,
\end{align*}
% \subsubsection{$\ell_1$-randomization}
% \evg[inline]{Arya, since we are using Lemma 19 for the proof of this Theorem, don't you need to add the condition $\alpha \geq 4\sqrt{\tfrac{2d^2}{T}}$?}
% \evg[inline]{After reading and re-reading, I understood that you do not actually use Lemma~19 in the current form. Need to modify it then to fit the proof.}
where {\color{purple}$m_{\ell_1} = \frac{(d-2)(d-1)}{2\bL{\bar{\tC}}_{d,1}d^2\kappa }$}, and again with the agreement that $[T_0 + 1, T] = \emptyset$ for all $T \leq T_0$.
\begin{theorem}[$\ell_1$-randomization]
\label{thm:sconvex_l1_uncons}
Let $f$ be an $\alpha$-strongly convex function. Consider the above parametrization for Algorithm \ref{algo:simplex}, and assume that $\bx_1$ is non-random. Let Assumptions \ref{nat} and \ref{ass1} hold. If ${\color{black}T \geq d^{2-\frac{\beta}{2}}}$, then  
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f^{\star}] \leq \cst_1\frac{d}{\alpha T}\norm{\bx_1-\bx^*}^{2}+\frac{\cst_2}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}\enspace,
\end{align*}
 with $\cst_1,\cst_2 > 0$ depend only on $\sigma^2, L, \bL, \beta$.
\end{theorem}


\paragraph{Proof strategy.}
For the case of $\com = \bbR^d$, both Theorems~\ref{thm:sconvex_l2_uncons} and~\ref{thm:sconvex_l1_uncons} are based on the following result, which is valid for a rather general class of gradient estimates.

\begin{lemma}\label{scuntunc}
    Consider the iterative algorithm defined in Eq.~\eqref{eq:algo_general}.
    Assume that $f$ is $\alpha$-strongly convex on $\mathbb{R}^d$.
    Assume that there exist two positive sequences $b_t, v_t : \bbN \to [0, \infty)$ and $m \in (0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    % \begin{align*}
    %     \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\left[\norm{\bg_t}^2 \mid \bx_t \right] \leq v_t + m \norm{\bx_t-\bx^*}^2\enspace.
    % \end{align*}
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2  \leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, we have for all $\bx \in \com$
    \begin{align*}
        \Exp[f(\bx_t)-f^{\star}]\leq \frac{r_t-r_{t+1}}{2\eta_t}-\frac{\alpha}{4}r_t+\frac{b_{t}^2}{\alpha}+\frac{\eta_t}{2}\big(v_t+m\Exp\|\nabla f (\bx_t)\|^2\big)\enspace,
    \end{align*}
    where $r_t = \Exp\|\bx_t - \bx^*\|^2$.
    % and $\bx_1 \in \mathbb{R}^d$, $\bx_{t + 1} = \bx_t - \eta_t \bg_t$ for all $t \geq 1$.
%     and $\alpha \geq 4\sqrt{\frac{2m}{T}}$. 
%     Then, by denoting  $T_0 = \floor{\frac{16m}{\alpha^2}}$ and $\bar{\bx}_{T_{0},T} = \frac{1}{T_{0}}\sum_{t=T_{0}+1}^{T}x_t$, we have
%     \begin{align}\nonumber
%     \Exp[f(\bar{\bx}_{T_{0},T})-f^{\star}] &\leq \frac{4m}{\alpha T}\norm{\bx_1 - \bx^*}^2 + \frac{2}{\alpha T}\sum_{t=1}^{T}\Big(b_t^2 + \frac{2}{t}v_t\Big).
% \end{align}
% where $\bx_1 \in \mathbb{R}^d$, $\bx_{t + 1} = \bx_t - \eta_t \bg_t$ for all $t \geq 1$,  with $\eta_{t} = \min\big(\frac{\alpha}{4m},\frac{4}{\alpha t}\big)$.
    
\end{lemma}

\subsubsection{Constrained optimization}
We now we assume that $\com \subset \bbR^d$ be a closed convex set. Consequently, since $f$ is continuously differentiable, its gradient is bounded on $\com$. This fact allows us to develop any-time results, that is, in the present part we do not require the knowledge of the optimization horizon $T$.
The results of this section are essentially corollaries of the following general result.
\begin{lemma}\label{scunt}
    Let $\com \subset \bbR^d$ be a closed convex set. 
    Assume that $f$ is $\alpha$-strongly convex on $\com$ and $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Consider the iterative algorithm in Eq.~\eqref{eq:algo_general}.
    Assume that there exist two positive sequences $b_t, v_t,  : \bbN \to [0, \infty)$ and $m \in [0, \infty)$ such that for all $t \geq 1$ it holds almost surely that
    \begin{align*}
        \norm{\Exp[\bg_t \mid \bx_t] - \nabla f(\bx_t)} \leq b_t\qquad\text{and}\qquad \Exp\norm{\bg_t}^2\leq v_t + m \Exp\norm{\nabla f(\bx_t)}^2\enspace.
    \end{align*}
    Then, for $\bar{\bx}_T = \tfrac{1}{T}\sum_{t = 1}^T \bx_t$ we have
    \begin{align*}
    \Exp[f(\bar\bx_T)-f^\star] \leq \frac{mG^2 \left(\log(T)+1\right)}{\alpha T}+ \frac{1}{\alpha T}\sum_{t=1}^{T}\left(\frac{v_t}{t}+b_t^2\right)\enspace,
\end{align*}


% where $\bx_1 \in \com$, $\bx_{t + 1} = \proj_{\com}(\bx_t - \eta_t \bg_t)$ for all $t \geq 1$ with $\eta_t = \tfrac{2}{\alpha t}$.
    
\end{lemma}
Using the bounds on the variance and bias derived in Section~\ref{sec3}, we can deduce the following two guarantees for Algorithms~\ref{algose} and~\ref{algo:simplex} by analysing the resulting recursive relations.


{\color{black} 
\begin{theorem}[$\ell_2$-randomization]
\label{thm:sconvex_l2_cons}
Let $f$ be an $\alpha$-strongly convex function. Let $\eta_t =\frac{2}{\alpha t}$ and $h_t = \left(\frac{d^2}{t}\right)^{\frac{1}{2\beta}}$ for Algorithm \ref{algose}, and assume that $\com$ is a convex and closed subset of $\mathbb{R}^d$, with $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Let Assumptions \ref{nat} and \ref{ass1} hold. Then  ,
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f(\bx)] &\leq \cst_1\frac{dG^2\left(\log(T)+1\right)}{\alpha T} +\frac{\cst_2}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}+\cst_3\frac{d^{1+\frac{2}{\beta}}}{\alpha T}\enspace,
\end{align*}
 with $\cst_1,\cst_2,\cst_3 > 0$ depend only on $\sigma^2, L, \bL, \beta$.
\end{theorem}
\begin{theorem}[$\ell_1$-randomization]
\label{thm:sconvex_l1_cons}
Let $f$ be an $\alpha$-strongly convex function. Let $\eta_t =\frac{2}{\alpha t}$ and $h_t = d^{\frac{2+\beta}{2\beta}}t^{-\frac{1}{2\beta}}$ for Algorithm \ref{algo:simplex}, and assume that $\com$ is a convex and closed subset of $\mathbb{R}^d$, with $\sup_{\bx \in \com} \|\nabla f(\bx)\|_2 \leq G$. Let Assumptions \ref{nat} and \ref{ass1} hold.Then,  
\begin{align*}
    \Exp[f(\bar{\bx}_T)-f^*] \leq \cst_1\frac{dG^2\left(\log(T)+1\right)}{\alpha T} +\frac{\cst_2}{\alpha}\left(\frac{d^2}{T}\right)^{\frac{\beta-1}{\beta}}+\cst_3\frac{d^{1+\frac{2}{\beta}}}{\alpha T}\enspace,
\end{align*}
 with $\cst_1,\cst_2, \cst_3 > 0$ depend only on $\sigma^2, L, \bL, \beta$.
\end{theorem}
}
The above results are nearly identical and they only differ in the exact values of constants $\cst_1, \cst_2, \cst_3$. Theorem~\ref{thm:sconvex_l2_cons} should be compared to~\cite[Theorem 4.1 and Theorem 5.1]{akhavan2020} and with~\cite[Theorem 1]{Gasnikov}. Note, however, both~\cite{akhavan2020,Gasnikov} work with a slightly different, compared to ours, notion of smoothness (both coincide in case $\beta = 2$, see our Remark~\ref{rem:smoothness}). The term $\tfrac{d^{1+2/\beta}}{T}$, appearing in both results is negligible as long as $T \geq d^{4 - \beta}$, which, in the worst case of $\beta = 2$ means that $T \geq d^2$.
\begin{remark}
Note that the condition on $d, T$ in this part is worse than in all the previously considered cases. Indeed, before we required $d^{2 - \sfrac{\beta}{2}}$, while here we have $d^{4 - \beta}$. Such an inflated condition is a consequence of the fact that in the present part the results are obtained \emph{without} the knowledge of the optimization horizon $T$, that is, Theorems~\ref{thm:sconvex_l2_cons} and~\ref{thm:sconvex_l1_cons} give anytime guarantees. Actually, one can relax the condition $d^{4 - \beta}$ back to $d^{2 - \sfrac{\beta}{2}}$ by assuming that $T$ is known and allowing $h_t$ to be dependent on $T$ (as we did in Theorems~\ref{thm:sconvex_l2_uncons} and~\ref{thm:sconvex_l1_uncons}). We do not further pursue this development.
\end{remark}
\evg[inline]{Arya, add a couple of words on why in the unconstrained case we have the condition $T \geq d^{2 - 2/\beta}$, while here it is $T \geq d^{4 - \beta}$}
\arya[inline]{The reason for the stronger condition on $T$ is that the choice of the parameters is independent of $T$. I don't know if we want to include the online result here or not. If we want to do so, it would be to assign the parameters for the online risk in which we insist not to make $\eta_t$ and $h_t$ dependent on $T$. Otherwise, I think there is no point in this and we can use similar techniques as in the proof of unconstrained case to have the same imposed condition on $T$.}
% Given the above result, the actual proofs of Theorems~\ref{thm:sconvex_l2_uncons} and~\ref{thm:sconvex_l1_uncons} amount to the substitution of the already discussed bounds on bias and variance of a given gradient estimate.

\begin{comment}
\begin{restatable}{theorem}{thdtheorem}
\label{thm:2}
	Let $f \in {\mathcal F}_{\alpha, \beta}(L)$ with $\alpha,L>0$ and $\beta \geq 2$.
	Let Assumptions \ref{nat} and \ref{ass1} hold and let $\com$ be a convex compact subset  of $\mathbb{R}^d$. Assume that $\max_{x\in\com}\|\nabla f(x)\|\le G $. %with Euclidean diameter ${\rm diam}(\com)\le B<\infty$.
	If $\sigma>0$ then the cumulative regret of Algorithm \ref{algo:grad} with \[h_t = \left(\frac{3\kappa\sigma^2}{2(\beta-1)(\kappa_\beta L)^2} \right)^{\frac{1}{2\beta}} t^{-\frac{1}{2\beta}},~~~\eta_t=\frac{2}{\alpha t},~~~t= 1,\dots,T~~~~~~~~\]  satisfies  
	\begin{equation}
	\label{eq:bound0}
	\forall x\in \com: \ \sum_{t=1}^T \Exp [ f(x_t) - f(x)]\le \frac{1}{\alpha}
	\left(
d \Big(A_1 T^{{1}/{\beta}}+A_2 \Big)
+  A_3   \log T
\right),
	\end{equation}
	where $A_1={3\beta}(\kappa\sigma^2)^{\frac{\beta-1}{\beta}}
(\kappa_\beta L)^{\frac{2}{\beta}}$, $A_2=\bar c {\bar L^2} (\sigma/L)^{\frac{2}{\beta}}+{9\kappa G^2}/{d}$ with constant $\bar c>0$ depending only on $\beta$, and $A_3 = 9 \kappa G^2$.
	The optimization error of averaged estimator ${\bar x}_T=\frac{1}{T}\sum_{t=1}^T x_t$ satisfies  
	\begin{equation}
	\label{eq:bound1}
	\Exp [ f({\bar x}_T) - f^*]\leq \frac{1}{\alpha}
\left(  d\left(\frac{A_1}{T^{\frac{\beta-1}{\beta}}}+ \frac{A_2}{T} \right)+ A_3 \,\frac{\log T}{T} \right).
		\end{equation}

			If $\sigma=0$, then the cumulative regret and the optimization error of Algorithm \ref{algo:grad} with any $h_t$ chosen small enough and $\eta_t=\frac{2}{\alpha t}$ satisfy the bounds \eqref{eq:bound0} and \eqref{eq:bound1}, respectively, with $A_1=0, A_2={9\kappa G^2}/{d}$ and $A_3=10\kappa G^2$. 
%		\begin{equation}
%	\label{eq:bound0a}
%	\forall x\in \com: \ \sum_{t=1}^T \Exp [ f(x_t) - f(x)]\le 10\kappa G^2  \,\frac{ d}{\alpha} \log T
%	\end{equation}
%	and
%	\begin{equation}
%	\label{eq:bound1a}
%	\Exp [ f({\bar x}_T) - f(x^*)]\leq 10\kappa G^2 \, \frac{ d}{\alpha}  \frac{\log T}{T}.
%		\end{equation}
\end{restatable}

\AK{
\begin{corollary}
Let $f:\mathbb{R}^d\to\mathbb{R}$ be a convex function belongs to $\mathcal{F}_{\beta}(L)$ with $L>0$ and $\beta \geq 2$. Let Assumptions \ref{nat} and \ref{ass1} hold and let $\com$ be a convex compact subset  of $\mathbb{R}^d$. Assume that $\max_{x\in\com}\|\nabla f(x)\|\le G $ and $\norm{x^*}^2 \leq \mathcal{B}^{'}$. %with Euclidean diameter ${\rm diam}(\com)\le B<\infty$.
	If $\sigma>0$, then the optimization error of Algorithm \ref{algo:grad} with \[h_t =  t^{-\frac{1}{2\beta}},~~~\eta_t=\frac{2}{\gamma t},~~~t= 1,\dots,T~~~~~~~~\]  satisfies 
	\begin{align*}
\Exp[f(\bar{x}_{T}) - f^*] \leq \mathcal{C}d^{1 - \frac{1}{2\beta}}T_{0}^{-\frac{\beta-1}{2\beta}}
	  \end{align*}
where $\mathcal{C}>0$ is a constant  depends only on $\sigma^2, L, \Bar{L}, \beta$, ${\bar x}_T=\frac{1}{T}\sum_{t=1}^T x_t$, $T_{0}$  is the total number of function evaluations, and $\gamma = d^{1-\frac{1}{2\beta}}T_{0}^{-\frac{\beta-1}{2\beta}}$.
\end{corollary}}
\begin{proof}
Consider the function $v: \mathbb{R}^{d} \to \mathbb{R}$, such that $v(x) = f(x) + \frac{\alpha}{2}\norm{x}^{2}$, where $\alpha >0$. It is clear that $v$ is an $\alpha$-strongly convex function. Therefore, by Theorem \ref{thm:1} we have
\begin{align*}
    \Exp[v(\bar{x}_{T}) - v^*] \leq \mathcal{C}_{1}\frac{d^{2 - \frac{1}{\beta}}}{\alpha}T_{0}^{-\frac{\beta-1}{\beta}},
\end{align*}
where $v^* = \argmin_{x \in \com}v(x)$, $\mathcal{C}_{1}>0$ and $T_{0}$ is the total number of function evaluations. By rearranging terms, we have
\begin{align*}
    \Exp[f(\bar{x}_{T}) - f^*] \leq \mathcal{C}_{1}\frac{d^{2 - \frac{1}{\beta}}}{\alpha}T_{0}^{-\frac{\beta-1}{\beta}}+\Exp[f(\bar{x}_{T})-v(\bar{x}_{T})] + v^* -f^*
\end{align*}
Now, since for each $x \in \mathbb{R}^d$, $f(x) \leq v(x)$, we have $\Exp[f(\bar{x}_{T})-v(\bar{x}_{T})] \leq 0$. On the other hand, $v^* \leq v(x^*)$, therefore $v^* - f^* \leq \frac{\alpha}{2}\mathcal{B}^{'}$. Letting $\alpha = d^{1- \frac{1}{2\beta}}T_{0}^{-\frac{\beta-1}{2\beta}}$, we get
\begin{align*}
    \Exp[f(\bar{x}_{T}) - f^*] \leq \mathcal{C}d^{(1 - \frac{1}{2\beta})}T_{0}^{-\frac{\beta-1}{2\beta}},
\end{align*}
where $\mathcal{C} = \mathcal{C}_{1} + \frac{\mathcal{B}^{'}}{2}.$
\end{proof}


% Now,  we consider the case $\beta=2$ and obtain improved bounds that scale as $d$ rather than $d^{\frac{3}{4}}$ with the dimension in the constrained optimization setting analogous to Theorem \ref{thm:1}. First note that for $\beta=2$ we can simplify the algorithm, outlined in Algorithm \ref{algo}. Instead of the inner loop Algorithm \ref{algo:grad}, we use the following gradient estimator
% \begin{equation}\label{gt}
%   \hat g_t = \frac{d}{2h_t} (y_t- y'_t) \zeta_t, 
% \end{equation}
% where $y_t=f(x_t+h_t \zeta_t)+\xi_t$ and $y'_t=f(x_t-h_t  \zeta_t) + \xi_t'$, and $\zeta_t$ is random vector uniformly distributed on the unit sphere  $S_d=\{u\in \mathbb{R}^d:\|u\|= 1 \}$. A well-known observation that goes back to \cite{NY1983} consists in the fact that $\hat g_t$ defined in \eqref{gt} is an unbiased estimator of the gradient at point $x_t$ of the surrogate function $\hat f_t$ defined by 
% \[
% \hat f_t(x)= \Exp f(x+h_t \tilde \zeta),\quad \forall x\in\mathbb{R}^d,
% \]
% where the expectation  $\Exp$ is taken   with respect to the random vector $\tilde \zeta$ uniformly distributed on the unit ball $\mathbb{B}_{d}=\{u\in \mathbb{R}^d:\|u\|\le 1 \}$.  The properties of the surrogate $\hat f_t$  are described in Lemmas \ref{lem6.2} and \ref{lem6.4} presented in the appendix.



% The improvement in the rate that we get for $\beta=2$ is due to the fact that we can consider Algorithm \ref{algo} with  $\hat g_t$ defined in \eqref{gt} as the SGD for the surrogate function. Then the bias of approximating $f$ by $\hat f_t$ scales as $h_t^2$, which is smaller than the squared bias of 
% approximating the gradient arising in the proof of Theorem \ref{thm:1} that scales as $d^2h_t^{2(\beta-1)}=d^2h_t^2$ when $\beta=2$. On the other hand, the stochastic variability terms are the same for both methods of proof. This explains the gain in dependency on $d$. However, this technique does not work for $\beta>2$ since then the error of approximating $f$ by $\hat f_t$, which is of the order $h_t
% ^\beta$ (with $h_t$ small), becomes too large compared to the bias $d^2h_t^{2(\beta-1)}$ of Theorem \ref{thm:1}. 
% %

% \begin{restatable}{theorem}{eiththeorem}
% \label{th6.3}
% Let $f\in \mathcal{F}_{\alpha, 2}(L)$ with $\alpha,L>0$.
% 	Let Assumption \ref{ass1}  hold and let $\com$ be a convex compact subset  of $\mathbb{R}^d$. Assume that $\max_{x\in\com}\|\nabla f(x)\|\le G $. 
% If $\sigma>0$ then for the updates $x_t$ as in item 3 of Algorithm \ref{algo} with $\hat g_t$ defined in \eqref{gt} and parameters $h_t= \left(\frac{3d^2\sigma^2}{4L\alpha t+9L^2d^2}\right)^{1/4}$ and $\eta_t = \frac{1}{\alpha t}$ we have 
% \begin{equation}\label{eq1:th6.3}
% \forall x\in \Theta: \ \ \Exp \sum_{t=1}^{T} \big(f(x_t) - f(x)\big)  
% \le  \min\left(GBT, 2\sqrt{3L}\sigma
% \frac{d}{\sqrt{\alpha}} \sqrt{T}+ A_4\frac{d^2}{\alpha} \log T\right), 
% \end{equation}
% where $B$ is the Euclidean diameter of $\com$ and 
% $A_4=
% %\frac{1}{2}\Big(  
% 6.5 L\sigma+ 22 G^2/d$. 
% %\Big)$.
% Moreover, if $x^*= \argmin_{x\in\com}f(x)$ the optimization error of averaged estimator ${\bar x}_T=\frac{1}{T}\sum_{t=1}^T x_t$ is bounded as  
% 	\begin{equation}
% 	\label{eq2:th6.3}
% 	\Exp [ f({\bar x}_T) - f(x^*)]\leq 
% 	\min\left(GB, 2\sqrt{3L}\sigma
%  \frac{d}{\sqrt{\alpha T}}+ A_4 \frac{d^2}{\alpha} \frac{\log T}{T}\right).
% 		\end{equation}
% Finally, if $\sigma=0$, then the cumulative regret of the same procedure $x_t$ with any $h_t>0$ chosen small enough and $\eta_t=\frac{1}{\alpha t}$ and the optimization error of its averaged version are of the order $\frac{d^2}{\alpha} \log T$ and $\frac{d^2}{\alpha} \frac{\log T}{T}$, respectively.                         \end{restatable}
% %\begin{remark}
% Note that the terms $\frac{d^2}{\alpha} \log T$ and $\frac{d^2}{\alpha} \frac{\log T}{T}$ appearing in these bounds can be improved to $\frac{d}{\alpha} \log T$ and $\frac{d}{\alpha} \frac{\log T}{T}$ at the expense of assuming that the norm $\|\nabla f\|$ is uniformly bounded by $G$ not only on $\com$ but also on a large enough Euclidean neighborhood of $\com$. Moreover, the $\log T$ factor in the bounds for the optimization error can be eliminated by considering averaging from $T/2$ to $T$ rather than from 1 to $T$ in the spirit of  \cite{rakhlin2011making}. We refer to the appendix %Theorems \ref{th6.3-bis} 
% for the details and proofs of these facts. A major conclusion is that, when $\sigma>0$ and we consider the optimization error,  those terms are negligible with respect to $d/\sqrt{\alpha T}$ and thus an attainable rate is $\min(1,d/\sqrt{\alpha T})$. 
% %\end{remark}

% %The online bound \eqref{eq1:th6.3} extends in an obvious way to the functions $f=f_t$ depending on $t$, cf. Remark \ref{rem32}. 
% %Having in mind the bandit setting,
% %\mas{This comment is probably going to be re-edited after we add the online regret and $f_t$ in th algorithm}
% We close this section by noting, in connection with the bandit setting, that the bound \eqref{eq1:th6.3} extends straightforwardly (up to a change in numerical constants) to the cumulative regret of the form $\Exp\sum_{t=1}^{T} \big(f_t(x_t\pm h_t\zeta_t) - f_t(x)\big)$, where the losses are measured at the query points and $f$ depends on $t$. This fact follows immediately from the proof of Theorem \ref{th6.3} presented in the appendix and the property \eqref{lem6.4_2}, see Lemma \ref{lem6.4} in the appendix.
\end{comment}
\subsection{Quadratic functions}
\label{sec:quadratic}
In this section we consider quadratic functions $f$. More precisely, we assume that the target function belongs to
\begin{align*}
    \mathcal{F}_{\quadr} \triangleq \enscond{f}{f(\bx) = \bx^{\top}\bfA\bx + \bb^{\top}\bx + c}\enspace,
\end{align*}
where $\bfA$ is a symmetric positive semi-definite matrix in $\mathbb{R}^{d \times d}$, $\bb \in \mathbb{R}^d$, and $c \in \mathbb{R}$.
Denote by $\lambda_{\max}(\bfA)$ and $\lambda_{\min}^{\nz}(\bfA)$ the largest and the smallest \emph{non-zero} eigenvalue of $\bfA$, respectively.
Define the effective dimension and the conditioning number of $\bfA$ as
\begin{align*}
    d_{\eff}(\bfA) \triangleq \frac{\tr(\bfA)}{\lambda_{\max}(\bfA)}\qquad\text{and}\qquad \mu(\bfA) \triangleq \frac{\lambda_{\max}(\bfA)}{\lambda_{\min}^{\nz}(\bfA)}\enspace,
\end{align*}
respectively. Note that the definition of the conditioning number differs from the more conventional one, where instead of the division by the smallest non-zero eigenvalue one divides by the smallest eigenvalue. In our case we do not assume that $\bfA$ is strictly positive definite. Hence, we rely on the definition above, which, unlike the conventional one, is always well defined.
Before stating the main result let us specify the choice of  a ``dummy'' kernel $K(\cdot)$ in Algorithms~\ref{algose} and~\ref{algo:simplex}, namely\footnote{For quadratic functions, the kernel and the randomization introduced by $r \in [-1, 1]$ are not necessary. However, in order to keep all the sections harmonized and avoid the introduction of another algorithm, we simply specify the ``dummy'' kernel above.}
\begin{align}
    \label{eq:dummy_kernel}
    K(r) =
    \begin{cases}
    1, &r \geq 0\\
    -1, &r < 0
    \end{cases}\enspace.
\end{align}
% \begin{align*}
%     \kappa_1 \triangleq \int_{-1}^1 r^2 K^2(r) \d r\qquad\text{and}\qquad \kappa_2 \triangleq \int_{-1}^1 K^2(r) \d r\enspace.
% \end{align*}
% We are in position to state the main result of this section.
% \AK{
% \paragraph{\texorpdfstring{$\ell_2$}{}-randomization}
\begin{theorem}[\texorpdfstring{$\ell_2$}{}-randomization]
\label{thm:upper_quadratic}
Assume that $f \in \mathcal{F}_{\quadr}$ and Assumption~\ref{ass1} is satisfied.
% Assume 
% Suppose that the biggest and the smallest \emph{non-zero} eigenvalues of $A$ are $\upsilon$ and $\gamma$, respectively.
Consider Algorithm~\ref{algose} with 
\[
\eta_t = \min \parent{\frac{1}{\tr(\bfA)},\, \frac{2}{\lambda_{\min}^{\nz}(\bfA) t}}\qquad\text{and}\qquad h_{t} = \sqrt{\frac{d}{\lambda_{\min}^{\nz}(\bfA)}} \enspace,
\]
$\com=\mathbb{R}^d$, and $K(\cdot)$ defined in Eq.~\eqref{eq:dummy_kernel}, and assume that $\bx_1$ is non-random.  %$\in \com$ 
Then,
\begin{align*}
    \Exp[f(\bx_T) - f^\star]\leq \frac{d_{\eff}(\bfA)}{\mu^{-1}(\bfA)}\cdot \frac{4}{T}\left(f(\bx_1) - f^\star + 8\sigma^2\right)\enspace.
\end{align*}

% \evg{Let's introduce the notation $f^\star$ instead of $f(\bx^*)$. In most of the cases we cannot guarantee the uniqueness of the solution.}
% where $\cst_{1} = 8 / 3$ and $\cst_{2} = 7\sigma^{2}/3$.
% Furthermore, 
% \begin{align}
%     \Exp[f(x_{T_{0}}) - f(x^*)]\leq \mathcal{C}\frac{d}{\gamma T_{0}}(f(x_1)-f(x^*) + \sigma^2),
% \end{align}
% where $T_{0}$ denotes the total number of function evaluations.
\end{theorem}
% }
% \arya[inline]{TO DO: Extend the result in Theorem  for $\Exp[\bx_T-\bx^*]$.}
% \paragraph{\texorpdfstring{$\ell_1$}{}-randomization.}
% \evg[inline]{TODO}
\begin{theorem}[\texorpdfstring{$\ell_1$}{}-randomization]
\label{thm:upper_quadraticl1}
Assume that $f \in \mathcal{F}_{\quadr}$ and Assumption~\ref{ass1} is satisfied.
% Assume 
% Suppose that the biggest and the smallest \emph{non-zero} eigenvalues of $A$ are $\upsilon$ and $\gamma$, respectively.
Consider Algorithm~\ref{algo:simplex} with 
\[
\eta_t = \min \parent{\frac{1}{2\tr(\bfA)},\, \frac{2}{\lambda_{\min}^{\nz}(\bfA) t}}\qquad\text{and}\qquad h_{t} = d\sqrt{\frac{2}{\lambda_{\min}^{\nz}(\bfA)}} \enspace,
\]
$\com=\mathbb{R}^d$, and $K(\cdot)$ defined in Eq.~\eqref{eq:dummy_kernel}, and assume that $\bx_1$ is non-random.  %$\in \com$ 
Then,

\begin{align*}
    \Exp[f(\bx_T) - f^\star]\leq \frac{d_{\eff}(\bfA)}{\mu^{-1}(\bfA)}\cdot \frac{8}{T}\left(f(\bx_1) - f^\star + 5\sigma^2\right)\enspace.
\end{align*}

% The proof is concluded.
% \evg{Let's introduce the notation $f^\star$ instead of $f(\bx^*)$. In most of the cases we cannot guarantee the uniqueness of the solution.}
% where $\cst_{1} = 8 / 3$ and $\cst_{2} = 7\sigma^{2}/3$.
% Furthermore, 
% \begin{align}
%     \Exp[f(x_{T_{0}}) - f(x^*)]\leq \mathcal{C}\frac{d}{\gamma T_{0}}(f(x_1)-f(x^*) + \sigma^2),
% \end{align}
% where $T_{0}$ denotes the total number of function evaluations.
\end{theorem}
We remark that both bound on this section involve four main parameters. First of all, the bounds scale linearly with the effective dimension $d_{\eff}(\bfA)$ instead of the ambient one $d$, which can be much lower. Secondly, we again emphasize that the notion of the conditioning number $\mu(\bfA)$ that we use is valid for any positive semi-definite matrix $\bfA$. Finally, the derived rate depends linearly on the quality of the initialization as well as the variance. \cite{Shamir13} provided an upper bound for the optimization of quadratic functions which scales as $d^2 / T$. Note, however, \cite{Shamir13} uses a different notion of noise, which is bounded by the squared norm of the query point.
